Kernel Density Estimation for Multiclass Quantification

Several disciplines, like the social sciences, epidemiology, sentiment analysis, or market research, are interested in knowing the distribution of the classes in a population rather than the individual labels of the members thereof. Quantification is the supervised machine learning task concerned with obtaining accurate predictors of class prevalence, and to do so particularly in the presence of label shift. The distribution-matching (DM) approaches represent one of the most important families among the quantification methods that have been proposed in the literature so far. Current DM approaches model the involved populations by means of histograms of posterior probabilities. In this paper, we argue that their application to the multiclass setting is suboptimal since the histograms become class-specific, thus missing the opportunity to model inter-class information that may exist in the data. We propose a new representation mechanism based on multivariate densities that we model via kernel density estimation (KDE). The experiments we have carried out show our method, dubbed KDEy, yields superior quantification performance with respect to previous DM approaches. We also investigate the KDE-based representation within the maximum likelihood framework and show KDEy often shows superior performance with respect to the expectation-maximization method for quantification, arguably the strongest contender in the quantification arena to date.

==> tables/tab_lequaT1A.tex <==

        \begin{tabular}{|c|c|c|c|c||c|c||c|c||c|c|c|} \cline{2-12}
        \multicolumn{1}{c|}{} & ACC & PACC & HDy & DM-T & DM-HD & KDEy-HD & DM-CS & KDEy-CS & DIR & EMQ & KDEy-ML \\\hline
LeQua-T1A (MAE) &  0.03133$^{\phantom{\ddag}}$ \cellcolor{red!35} &  0.02642$^{\phantom{\ddag}}$ \cellcolor{green!8} &  0.02660$^{\phantom{\ddag}}$ \cellcolor{green!7} &  0.02364$^{\dag}$ \cellcolor{green!33} &  0.02371$^{\phantom{\ddag}}$ \cellcolor{green!33} & \textbf{0.02350}$^{\phantom{\ddag}}$ \cellcolor{green!35} &  0.02502$^{\phantom{\ddag}}$ \cellcolor{green!21} &  0.02473$^{\phantom{\ddag}}$ \cellcolor{green!23} &  0.02463$^{\phantom{\ddag}}$ \cellcolor{green!24} &  0.02359$^{\ddag}$ \cellcolor{green!34} &  0.02417$^{\phantom{\ddag}}$ \cellcolor{green!29} \\\hline
LeQua-T1A (MRAE) &  0.18025$^{\phantom{\ddag}}$ \cellcolor{red!35} &  0.16476$^{\phantom{\ddag}}$ \cellcolor{red!19} &  0.15654$^{\phantom{\ddag}}$ \cellcolor{red!11} &  0.12019$^{\phantom{\ddag}}$ \cellcolor{green!23} &  0.11711$^{\phantom{\ddag}}$ \cellcolor{green!26} &  0.11766$^{\phantom{\ddag}}$ \cellcolor{green!26} &  0.14913$^{\phantom{\ddag}}$ \cellcolor{red!4} &  0.14167$^{\phantom{\ddag}}$ \cellcolor{green!2} &  0.13777$^{\phantom{\ddag}}$ \cellcolor{green!6} & \textbf{0.10878}$^{\phantom{\ddag}}$ \cellcolor{green!35} &  0.11641$^{\phantom{\ddag}}$ \cellcolor{green!27} \\\hline
\end{tabular}

==> tables/tab_lequaT1B.tex <==

        \begin{tabular}{|c|c|c|c|c||c|c||c|c||c|c|c|} \cline{2-12}
        \multicolumn{1}{c|}{} & ACC & PACC & HDy-OvA & DM-T & DM-HD & KDEy-HD & DM-CS & KDEy-CS & DIR & EMQ & KDEy-ML \rule{0pt}{10pt}   \\\hline
LeQua-T1B (MAE) &  0.02081$^{\phantom{\ddag}}$ \cellcolor{red!21} &  0.01277$^{\phantom{\ddag}}$ \cellcolor{green!19} &  0.02331$^{\phantom{\ddag}}$ \cellcolor{red!35} &  0.01070$^{\phantom{\ddag}}$ \cellcolor{green!30} &  0.01112$^{\phantom{\ddag}}$ \cellcolor{green!28} & \textbf{0.00984}$^{\phantom{\ddag}}$ \cellcolor{green!35} &  0.01336$^{\phantom{\ddag}}$ \cellcolor{green!16} &  0.00996$^{\phantom{\ddag}}$ \cellcolor{green!34} &  0.01546$^{\phantom{\ddag}}$ \cellcolor{green!5} &  0.01177$^{\phantom{\ddag}}$ \cellcolor{green!24} &  0.01153$^{\phantom{\ddag}}$ \cellcolor{green!26} \\\hline
LeQua-T1B (MRAE) &  1.72371$^{\phantom{\ddag}}$ \cellcolor{red!16} &  1.37638$^{\phantom{\ddag}}$ \cellcolor{green!2} &  2.04481$^{\phantom{\ddag}}$ \cellcolor{red!35} &  0.92422$^{\phantom{\ddag}}$ \cellcolor{green!28} &  0.91116$^{\phantom{\ddag}}$ \cellcolor{green!29} & \textbf{0.81013}$^{\phantom{\ddag}}$ \cellcolor{green!35} &  1.73593$^{\phantom{\ddag}}$ \cellcolor{red!17} &  0.84367$^{\phantom{\ddag}}$ \cellcolor{green!33} &  1.97045$^{\phantom{\ddag}}$ \cellcolor{red!30} &  0.87802$^{\phantom{\ddag}}$ \cellcolor{green!31} &  0.82795$^{\phantom{\ddag}}$ \cellcolor{green!33} \\\hline

\end{tabular}

==> tables/tab_tweet_mae.tex <==

            \begin{tabular}{|c|c|c|c|c||c|c||c|c||c|c|c|} \cline{2-12}
            \multicolumn{1}{c}{} & 
            \multicolumn{2}{|c}{Adjustment} & 
            \multicolumn{6}{|c|}{Distribution Matching} & 
            \multicolumn{3}{c|}{Maximum Likelihood} \\
             \cline{2-12} 
            \multicolumn{1}{c|}{} & ACC & PACC & HDy-OvA & DM-T & DM-HD & KDEy-HD & DM-CS & KDEy-CS & DIR & EMQ & KDEy-ML \rule{0pt}{10pt}   \\\hline
gasp & .0575$^{\phantom{\ddag}}$ \cellcolor{red!0} & .0427$^{\phantom{\ddag}}$ \cellcolor{green!25} & .0774$^{\phantom{\ddag}}$ \cellcolor{red!35} & .0403$^{\phantom{\ddag}}$ \cellcolor{green!29} & .0398$^{\phantom{\ddag}}$ \cellcolor{green!30} & .0382$^{\dag}$ \cellcolor{green!33} & .0464$^{\phantom{\ddag}}$ \cellcolor{green!19} & .0420$^{\phantom{\ddag}}$ \cellcolor{green!26} & .0540$^{\phantom{\ddag}}$ \cellcolor{green!5} & .0447$^{\phantom{\ddag}}$ \cellcolor{green!21} & \textbf{.0372}$^{\phantom{\ddag}}$ \cellcolor{green!35} \\\hline
hcr & .1037$^{\phantom{\ddag}}$ \cellcolor{green!3} & .0714$^{\phantom{\ddag}}$ \cellcolor{green!32} & .1458$^{\phantom{\ddag}}$ \cellcolor{red!35} & .0869$^{\phantom{\ddag}}$ \cellcolor{green!18} & .0831$^{\phantom{\ddag}}$ \cellcolor{green!21} & .0726$^{\phantom{\ddag}}$ \cellcolor{green!31} & .0760$^{\phantom{\ddag}}$ \cellcolor{green!28} & .0798$^{\phantom{\ddag}}$ \cellcolor{green!24} & .0716$^{\ddag}$ \cellcolor{green!32} & .0787$^{\phantom{\ddag}}$ \cellcolor{green!25} & \textbf{.0688}$^{\phantom{\ddag}}$ \cellcolor{green!35} \\\hline
omd & .0769$^{\phantom{\ddag}}$ \cellcolor{green!5} & .0616$^{\phantom{\ddag}}$ \cellcolor{green!28} & .1036$^{\phantom{\ddag}}$ \cellcolor{red!35} & .0775$^{\phantom{\ddag}}$ \cellcolor{green!4} & .0616$^{\phantom{\ddag}}$ \cellcolor{green!28} & \textbf{.0570}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .0680$^{\phantom{\ddag}}$ \cellcolor{green!18} & .0665$^{\phantom{\ddag}}$ \cellcolor{green!20} & .0626$^{\phantom{\ddag}}$ \cellcolor{green!26} & .0608$^{\phantom{\ddag}}$ \cellcolor{green!29} & .0610$^{\phantom{\ddag}}$ \cellcolor{green!29} \\\hline
Sanders & .0733$^{\phantom{\ddag}}$ \cellcolor{green!11} & .0510$^{\phantom{\ddag}}$ \cellcolor{green!26} & .1410$^{\phantom{\ddag}}$ \cellcolor{red!35} & .0493$^{\phantom{\ddag}}$ \cellcolor{green!28} & .0495$^{\phantom{\ddag}}$ \cellcolor{green!28} & \textbf{.0394}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .0442$^{\phantom{\ddag}}$ \cellcolor{green!31} & .0460$^{\phantom{\ddag}}$ \cellcolor{green!30} & .0851$^{\phantom{\ddag}}$ \cellcolor{green!3} & .0448$^{\phantom{\ddag}}$ \cellcolor{green!31} & .0399$^{\ddag}$ \cellcolor{green!34} \\\hline
SemEval13 & .0819$^{\phantom{\ddag}}$ \cellcolor{green!16} & .0727$^{\phantom{\ddag}}$ \cellcolor{green!27} & .1223$^{\phantom{\ddag}}$ \cellcolor{red!35} & .0706$^{\phantom{\ddag}}$ \cellcolor{green!30} & .0708$^{\phantom{\ddag}}$ \cellcolor{green!30} & \textbf{.0669}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .0764$^{\phantom{\ddag}}$ \cellcolor{green!23} & .0680$^{\ddag}$ \cellcolor{green!33} & .1048$^{\phantom{\ddag}}$ \cellcolor{red!12} & .0949$^{\phantom{\ddag}}$ \cellcolor{red!0} & .0679$^{\dag}$ \cellcolor{green!33} \\\hline
SemEval14 & .0660$^{\phantom{\ddag}}$ \cellcolor{green!12} & .0581$^{\phantom{\ddag}}$ \cellcolor{green!25} & .0939$^{\phantom{\ddag}}$ \cellcolor{red!35} & .0549$^{\phantom{\ddag}}$ \cellcolor{green!31} & .0579$^{\phantom{\ddag}}$ \cellcolor{green!26} & \textbf{.0528}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .0608$^{\phantom{\ddag}}$ \cellcolor{green!21} & .0622$^{\phantom{\ddag}}$ \cellcolor{green!18} & .0825$^{\phantom{\ddag}}$ \cellcolor{red!15} & .0752$^{\phantom{\ddag}}$ \cellcolor{red!3} & .0601$^{\phantom{\ddag}}$ \cellcolor{green!22} \\\hline
SemEval15 & .1047$^{\phantom{\ddag}}$ \cellcolor{red!15} & .0917$^{\phantom{\ddag}}$ \cellcolor{green!18} & .1122$^{\phantom{\ddag}}$ \cellcolor{red!35} & .0899$^{\phantom{\ddag}}$ \cellcolor{green!22} & .0911$^{\phantom{\ddag}}$ \cellcolor{green!19} & .0875$^{\phantom{\ddag}}$ \cellcolor{green!28} & .0914$^{\phantom{\ddag}}$ \cellcolor{green!18} & .0862$^{\ddag}$ \cellcolor{green!32} & .1100$^{\phantom{\ddag}}$ \cellcolor{red!29} & .0985$^{\phantom{\ddag}}$ \cellcolor{green!0} & \textbf{.0852}$^{\phantom{\ddag}}$ \cellcolor{green!35} \\\hline
SemEval16 & .1380$^{\phantom{\ddag}}$ \cellcolor{red!4} & .1126$^{\phantom{\ddag}}$ \cellcolor{green!22} & .1674$^{\phantom{\ddag}}$ \cellcolor{red!35} & .1365$^{\phantom{\ddag}}$ \cellcolor{red!2} & .1361$^{\phantom{\ddag}}$ \cellcolor{red!1} & .1238$^{\phantom{\ddag}}$ \cellcolor{green!10} & .1494$^{\phantom{\ddag}}$ \cellcolor{red!16} & .1364$^{\phantom{\ddag}}$ \cellcolor{red!2} & .1211$^{\phantom{\ddag}}$ \cellcolor{green!13} & \textbf{.1010}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .1205$^{\phantom{\ddag}}$ \cellcolor{green!14} \\\hline
sst & .0698$^{\phantom{\ddag}}$ \cellcolor{red!14} & .0587$^{\phantom{\ddag}}$ \cellcolor{green!19} & .0766$^{\phantom{\ddag}}$ \cellcolor{red!35} & .0563$^{\phantom{\ddag}}$ \cellcolor{green!27} & .0565$^{\phantom{\ddag}}$ \cellcolor{green!26} & .0563$^{\phantom{\ddag}}$ \cellcolor{green!27} & .0600$^{\phantom{\ddag}}$ \cellcolor{green!15} & .0595$^{\phantom{\ddag}}$ \cellcolor{green!17} & .0641$^{\phantom{\ddag}}$ \cellcolor{green!3} & .0557$^{\dag}$ \cellcolor{green!29} & \textbf{.0538}$^{\phantom{\ddag}}$ \cellcolor{green!35} \\\hline
wa & .0521$^{\phantom{\ddag}}$ \cellcolor{red!35} & .0454$^{\phantom{\ddag}}$ \cellcolor{red!4} & .0466$^{\phantom{\ddag}}$ \cellcolor{red!10} & .0375$^{\phantom{\ddag}}$ \cellcolor{green!30} & .0377$^{\phantom{\ddag}}$ \cellcolor{green!30} & .0400$^{\phantom{\ddag}}$ \cellcolor{green!19} & .0425$^{\phantom{\ddag}}$ \cellcolor{green!8} & .0388$^{\phantom{\ddag}}$ \cellcolor{green!25} & .0432$^{\phantom{\ddag}}$ \cellcolor{green!4} & .0391$^{\phantom{\ddag}}$ \cellcolor{green!23} & \textbf{.0366}$^{\phantom{\ddag}}$ \cellcolor{green!35} \\\hline
wb & .0482$^{\phantom{\ddag}}$ \cellcolor{red!3} & .0461$^{\phantom{\ddag}}$ \cellcolor{green!1} & .0600$^{\phantom{\ddag}}$ \cellcolor{red!35} & .0355$^{\phantom{\ddag}}$ \cellcolor{green!30} & .0355$^{\phantom{\ddag}}$ \cellcolor{green!30} & .0348$^{\phantom{\ddag}}$ \cellcolor{green!32} & .0388$^{\phantom{\ddag}}$ \cellcolor{green!21} & .0396$^{\phantom{\ddag}}$ \cellcolor{green!19} & .0473$^{\phantom{\ddag}}$ \cellcolor{red!1} & \textbf{.0337}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .0351$^{\phantom{\ddag}}$ \cellcolor{green!31} \\\hline
\hline
Ave (MAE) & .0793$^{\phantom{\ddag}}$ \cellcolor{green!4} & .0647$^{\phantom{\ddag}}$ \cellcolor{green!28} & .1042$^{\phantom{\ddag}}$ \cellcolor{red!35} & .0668$^{\phantom{\ddag}}$ \cellcolor{green!24} & .0654$^{\phantom{\ddag}}$ \cellcolor{green!27} & .0609$^{\phantom{\ddag}}$ \cellcolor{green!34} & .0685$^{\phantom{\ddag}}$ \cellcolor{green!22} & .0659$^{\phantom{\ddag}}$ \cellcolor{green!26} & .0769$^{\phantom{\ddag}}$ \cellcolor{green!8} & .0661$^{\phantom{\ddag}}$ \cellcolor{green!26} & \textbf{.0605}$^{\phantom{\ddag}}$ \cellcolor{green!35} \\\hline

\end{tabular}

==> tables/tab_tweet_mrae.tex <==

            \begin{tabular}{|c|c|c|c|c||c|c||c|c||c|c|c|} \cline{2-12}
            \multicolumn{1}{c}{} & 
            \multicolumn{2}{|c}{Adjustment} & 
            \multicolumn{6}{|c|}{Distribution Matching} & 
            \multicolumn{3}{c|}{Maximum Likelihood} \\
             \cline{2-12} 
            \multicolumn{1}{c|}{} & ACC & PACC & HDy-OvA & DM-T & DM-HD & KDEy-HD & DM-CS & KDEy-CS & DIR & EMQ & KDEy-ML \rule{0pt}{10pt}   \\\hline
gasp &  0.3723$^{\phantom{\ddag}}$ \cellcolor{red!8} &  0.2933$^{\phantom{\ddag}}$ \cellcolor{green!20} &  0.4446$^{\phantom{\ddag}}$ \cellcolor{red!35} &  0.3287$^{\phantom{\ddag}}$ \cellcolor{green!7} &  0.2893$^{\phantom{\ddag}}$ \cellcolor{green!22} &  0.2744$^{\dag}$ \cellcolor{green!27} &  0.3557$^{\phantom{\ddag}}$ \cellcolor{red!2} &  0.2785$^{\ddag}$ \cellcolor{green!26} &  0.4295$^{\phantom{\ddag}}$ \cellcolor{red!29} &  0.3591$^{\phantom{\ddag}}$ \cellcolor{red!3} & \textbf{0.2550}$^{\phantom{\ddag}}$ \cellcolor{green!35} \\\hline
hcr &  0.8680$^{\phantom{\ddag}}$ \cellcolor{red!35} &  0.7948$^{\phantom{\ddag}}$ \cellcolor{red!22} &  0.6668$^{\phantom{\ddag}}$ \cellcolor{red!1} &  0.5952$^{\phantom{\ddag}}$ \cellcolor{green!10} &  0.6386$^{\phantom{\ddag}}$ \cellcolor{green!2} &  0.5521$^{\phantom{\ddag}}$ \cellcolor{green!17} &  0.5657$^{\phantom{\ddag}}$ \cellcolor{green!15} &  0.5595$^{\phantom{\ddag}}$ \cellcolor{green!16} &  0.4548$^{\phantom{\ddag}}$ \cellcolor{green!33} & \textbf{0.4452}$^{\phantom{\ddag}}$ \cellcolor{green!35} &  0.4685$^{\ddag}$ \cellcolor{green!31} \\\hline
omd &  0.5697$^{\phantom{\ddag}}$ \cellcolor{red!19} &  0.4273$^{\phantom{\ddag}}$ \cellcolor{green!12} &  0.6386$^{\phantom{\ddag}}$ \cellcolor{red!35} &  0.6189$^{\phantom{\ddag}}$ \cellcolor{red!30} &  0.3781$^{\phantom{\ddag}}$ \cellcolor{green!23} &  0.3416$^{\phantom{\ddag}}$ \cellcolor{green!31} &  0.4877$^{\phantom{\ddag}}$ \cellcolor{red!1} &  0.4186$^{\phantom{\ddag}}$ \cellcolor{green!13} &  0.5185$^{\phantom{\ddag}}$ \cellcolor{red!8} &  0.3950$^{\phantom{\ddag}}$ \cellcolor{green!19} & \textbf{0.3243}$^{\phantom{\ddag}}$ \cellcolor{green!35} \\\hline
Sanders &  0.4051$^{\phantom{\ddag}}$ \cellcolor{green!1} &  0.3633$^{\phantom{\ddag}}$ \cellcolor{green!9} &  0.5633$^{\phantom{\ddag}}$ \cellcolor{red!31} &  0.3056$^{\phantom{\ddag}}$ \cellcolor{green!21} &  0.2627$^{\phantom{\ddag}}$ \cellcolor{green!30} & \textbf{0.2425}$^{\phantom{\ddag}}$ \cellcolor{green!35} &  0.2665$^{\phantom{\ddag}}$ \cellcolor{green!30} &  0.2675$^{\phantom{\ddag}}$ \cellcolor{green!29} &  0.5800$^{\phantom{\ddag}}$ \cellcolor{red!35} &  0.2810$^{\phantom{\ddag}}$ \cellcolor{green!27} &  0.2604$^{\phantom{\ddag}}$ \cellcolor{green!31} \\\hline
SemEval13 &  0.5541$^{\phantom{\ddag}}$ \cellcolor{green!8} &  0.5086$^{\phantom{\ddag}}$ \cellcolor{green!17} &  0.7922$^{\phantom{\ddag}}$ \cellcolor{red!35} &  0.4360$^{\phantom{\ddag}}$ \cellcolor{green!30} &  0.4495$^{\phantom{\ddag}}$ \cellcolor{green!28} &  0.4402$^{\phantom{\ddag}}$ \cellcolor{green!29} &  0.4901$^{\phantom{\ddag}}$ \cellcolor{green!20} &  0.4276$^{\ddag}$ \cellcolor{green!32} &  0.7031$^{\phantom{\ddag}}$ \cellcolor{red!18} &  0.6605$^{\phantom{\ddag}}$ \cellcolor{red!10} & \textbf{0.4122}$^{\phantom{\ddag}}$ \cellcolor{green!35} \\\hline
SemEval14 &  0.4948$^{\phantom{\ddag}}$ \cellcolor{green!7} &  0.4541$^{\dag}$ \cellcolor{green!18} &  0.6473$^{\phantom{\ddag}}$ \cellcolor{red!35} &  0.4125$^{\phantom{\ddag}}$ \cellcolor{green!30} &  0.4020$^{\phantom{\ddag}}$ \cellcolor{green!33} &  0.4048$^{\phantom{\ddag}}$ \cellcolor{green!32} &  0.4781$^{\phantom{\ddag}}$ \cellcolor{green!12} &  0.4063$^{\phantom{\ddag}}$ \cellcolor{green!32} &  0.5621$^{\phantom{\ddag}}$ \cellcolor{red!11} &  0.5733$^{\phantom{\ddag}}$ \cellcolor{red!14} & \textbf{0.3955}$^{\phantom{\ddag}}$ \cellcolor{green!35} \\\hline
SemEval15 &  0.6975$^{\phantom{\ddag}}$ \cellcolor{green!3} &  0.6687$^{\phantom{\ddag}}$ \cellcolor{green!11} &  0.8367$^{\phantom{\ddag}}$ \cellcolor{red!35} &  0.6008$^{\phantom{\ddag}}$ \cellcolor{green!30} &  0.6019$^{\phantom{\ddag}}$ \cellcolor{green!30} &  0.6110$^{\phantom{\ddag}}$ \cellcolor{green!27} &  0.6361$^{\phantom{\ddag}}$ \cellcolor{green!20} &  0.6022$^{\ddag}$ \cellcolor{green!30} &  0.7996$^{\phantom{\ddag}}$ \cellcolor{red!24} &  0.7577$^{\phantom{\ddag}}$ \cellcolor{red!12} & \textbf{0.5858}$^{\phantom{\ddag}}$ \cellcolor{green!35} \\\hline
SemEval16 &  1.1051$^{\phantom{\ddag}}$ \cellcolor{green!2} &  0.9638$^{\ddag}$ \cellcolor{green!15} &  1.0624$^{\phantom{\ddag}}$ \cellcolor{green!6} &  0.8354$^{\dag}$ \cellcolor{green!27} &  0.8114$^{\phantom{\ddag}}$ \cellcolor{green!29} & \textbf{0.7557}$^{\phantom{\ddag}}$ \cellcolor{green!35} &  0.8435$^{\phantom{\ddag}}$ \cellcolor{green!26} &  0.9716$^{\phantom{\ddag}}$ \cellcolor{green!15} &  1.5153$^{\phantom{\ddag}}$ \cellcolor{red!35} &  0.9803$^{\ddag}$ \cellcolor{green!14} &  0.7668$^{\ddag}$ \cellcolor{green!33} \\\hline
sst &  0.5427$^{\phantom{\ddag}}$ \cellcolor{red!35} &  0.4717$^{\phantom{\ddag}}$ \cellcolor{red!9} &  0.4135$^{\phantom{\ddag}}$ \cellcolor{green!12} &  0.3750$^{\phantom{\ddag}}$ \cellcolor{green!26} &  0.3594$^{\phantom{\ddag}}$ \cellcolor{green!32} &  0.4117$^{\phantom{\ddag}}$ \cellcolor{green!12} &  0.4218$^{\phantom{\ddag}}$ \cellcolor{green!9} &  0.4634$^{\phantom{\ddag}}$ \cellcolor{red!5} &  0.4834$^{\phantom{\ddag}}$ \cellcolor{red!13} &  0.4446$^{\phantom{\ddag}}$ \cellcolor{green!0} & \textbf{0.3514}$^{\phantom{\ddag}}$ \cellcolor{green!35} \\\hline
wa &  0.3214$^{\phantom{\ddag}}$ \cellcolor{red!35} &  0.2995$^{\phantom{\ddag}}$ \cellcolor{red!20} &  0.2920$^{\phantom{\ddag}}$ \cellcolor{red!15} & \textbf{0.2142}$^{\phantom{\ddag}}$ \cellcolor{green!35} &  0.2213$^{\phantom{\ddag}}$ \cellcolor{green!30} &  0.2682$^{\phantom{\ddag}}$ \cellcolor{red!0} &  0.3017$^{\phantom{\ddag}}$ \cellcolor{red!22} &  0.2333$^{\ddag}$ \cellcolor{green!22} &  0.2726$^{\phantom{\ddag}}$ \cellcolor{red!3} &  0.2238$^{\ddag}$ \cellcolor{green!28} &  0.2320$^{\ddag}$ \cellcolor{green!23} \\\hline
wb &  0.3373$^{\phantom{\ddag}}$ \cellcolor{red!35} &  0.3112$^{\phantom{\ddag}}$ \cellcolor{red!20} &  0.3087$^{\phantom{\ddag}}$ \cellcolor{red!19} &  0.2417$^{\phantom{\ddag}}$ \cellcolor{green!17} &  0.2330$^{\phantom{\ddag}}$ \cellcolor{green!22} &  0.2261$^{\phantom{\ddag}}$ \cellcolor{green!26} &  0.2719$^{\phantom{\ddag}}$ \cellcolor{green!0} &  0.2575$^{\phantom{\ddag}}$ \cellcolor{green!8} &  0.2426$^{\phantom{\ddag}}$ \cellcolor{green!17} & \textbf{0.2099}$^{\phantom{\ddag}}$ \cellcolor{green!35} &  0.2202$^{\phantom{\ddag}}$ \cellcolor{green!29} \\\hline
\hline
Ave (MRAE) &  0.5698$^{\phantom{\ddag}}$ \cellcolor{red!23} &  0.5051$^{\phantom{\ddag}}$ \cellcolor{red!2} &  0.6060$^{\phantom{\ddag}}$ \cellcolor{red!35} &  0.4513$^{\phantom{\ddag}}$ \cellcolor{green!14} &  0.4225$^{\phantom{\ddag}}$ \cellcolor{green!24} &  0.4117$^{\phantom{\ddag}}$ \cellcolor{green!27} &  0.4653$^{\phantom{\ddag}}$ \cellcolor{green!10} &  0.4442$^{\phantom{\ddag}}$ \cellcolor{green!17} &  0.5965$^{\phantom{\ddag}}$ \cellcolor{red!31} &  0.4846$^{\phantom{\ddag}}$ \cellcolor{green!4} & \textbf{0.3884}$^{\phantom{\ddag}}$ \cellcolor{green!35} \\\hline

\end{tabular}

==> tables/tab_uci_mae.tex <==

            \begin{tabular}{|c|c|c|c|c||c|c||c|c||c|c|c|} \cline{2-12}
            \multicolumn{1}{c}{} & 
            \multicolumn{2}{|c}{Adjustment} & 
            \multicolumn{6}{|c|}{Distribution Matching} & 
            \multicolumn{3}{c|}{Maximum Likelihood} \\
             \cline{2-12} 
            \multicolumn{1}{c|}{} & ACC & PACC & HDy & DM-T & DM-HD & KDEy-HD & DM-CS & KDEy-CS & DIR & EMQ & KDEy-ML \\\hline
balance.1 & .0177$^{\phantom{\ddag}}$ \cellcolor{green!24} & \textbf{.0113}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .0193$^{\phantom{\ddag}}$ \cellcolor{green!21} & .0136$^{\phantom{\ddag}}$ \cellcolor{green!31} & .0192$^{\phantom{\ddag}}$ \cellcolor{green!21} & .0215$^{\phantom{\ddag}}$ \cellcolor{green!17} & .0371$^{\phantom{\ddag}}$ \cellcolor{red!8} & .0527$^{\phantom{\ddag}}$ \cellcolor{red!35} & .0138$^{\phantom{\ddag}}$ \cellcolor{green!30} & .0203$^{\phantom{\ddag}}$ \cellcolor{green!19} & .0183$^{\phantom{\ddag}}$ \cellcolor{green!23} \\\cline{2-12}
balance.3 & .0238$^{\phantom{\ddag}}$ \cellcolor{red!6} & .0186$^{\phantom{\ddag}}$ \cellcolor{green!26} & .0179$^{\ddag}$ \cellcolor{green!30} & .0285$^{\phantom{\ddag}}$ \cellcolor{red!35} & .0189$^{\phantom{\ddag}}$ \cellcolor{green!24} & .0211$^{\phantom{\ddag}}$ \cellcolor{green!10} & .0240$^{\phantom{\ddag}}$ \cellcolor{red!6} & .0242$^{\phantom{\ddag}}$ \cellcolor{red!8} & \textbf{.0172}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .0242$^{\phantom{\ddag}}$ \cellcolor{red!8} & .0237$^{\phantom{\ddag}}$ \cellcolor{red!5} \\\cline{2-12}
breast-cancer & .0276$^{\phantom{\ddag}}$ \cellcolor{red!6} & .0236$^{\phantom{\ddag}}$ \cellcolor{green!2} & .0411$^{\phantom{\ddag}}$ \cellcolor{red!35} & .0173$^{\phantom{\ddag}}$ \cellcolor{green!15} & .0243$^{\phantom{\ddag}}$ \cellcolor{green!0} & .0203$^{\phantom{\ddag}}$ \cellcolor{green!9} & .0098$^{\phantom{\ddag}}$ \cellcolor{green!31} & \textbf{.0080}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .0127$^{\phantom{\ddag}}$ \cellcolor{green!24} & .0090$^{\phantom{\ddag}}$ \cellcolor{green!32} & .0131$^{\phantom{\ddag}}$ \cellcolor{green!24} \\\cline{2-12}
cmc.1 & .0896$^{\phantom{\ddag}}$ \cellcolor{green!25} & .0862$^{\dag}$ \cellcolor{green!28} & .1543$^{\phantom{\ddag}}$ \cellcolor{red!35} & .0940$^{\phantom{\ddag}}$ \cellcolor{green!21} & .0962$^{\phantom{\ddag}}$ \cellcolor{green!19} & .0922$^{\phantom{\ddag}}$ \cellcolor{green!23} & .1218$^{\phantom{\ddag}}$ \cellcolor{red!4} & .1037$^{\phantom{\ddag}}$ \cellcolor{green!12} & \textbf{.0796}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .0912$^{\phantom{\ddag}}$ \cellcolor{green!24} & .0974$^{\phantom{\ddag}}$ \cellcolor{green!18} \\\cline{2-12}
cmc.2 & .0987$^{\phantom{\ddag}}$ \cellcolor{green!23} & .1011$^{\phantom{\ddag}}$ \cellcolor{green!22} & .2712$^{\phantom{\ddag}}$ \cellcolor{red!35} & .1777$^{\phantom{\ddag}}$ \cellcolor{red!3} & .1837$^{\phantom{\ddag}}$ \cellcolor{red!5} & .0861$^{\phantom{\ddag}}$ \cellcolor{green!27} & .0864$^{\phantom{\ddag}}$ \cellcolor{green!27} & .0788$^{\phantom{\ddag}}$ \cellcolor{green!29} & \textbf{.0634}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .0700$^{\phantom{\ddag}}$ \cellcolor{green!32} & .0879$^{\phantom{\ddag}}$ \cellcolor{green!26} \\\cline{2-12}
cmc.3 & .1461$^{\phantom{\ddag}}$ \cellcolor{red!31} & .1399$^{\phantom{\ddag}}$ \cellcolor{red!22} & .1078$^{\ddag}$ \cellcolor{green!25} & .1300$^{\phantom{\ddag}}$ \cellcolor{red!7} & .1216$^{\phantom{\ddag}}$ \cellcolor{green!5} & .1238$^{\phantom{\ddag}}$ \cellcolor{green!1} & .1435$^{\phantom{\ddag}}$ \cellcolor{red!27} & .1483$^{\phantom{\ddag}}$ \cellcolor{red!35} & \textbf{.1018}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .1272$^{\phantom{\ddag}}$ \cellcolor{red!3} & .1233$^{\phantom{\ddag}}$ \cellcolor{green!2} \\\cline{2-12}
ctg.1 & .0307$^{\phantom{\ddag}}$ \cellcolor{red!35} & .0192$^{\phantom{\ddag}}$ \cellcolor{green!15} & .0169$^{\phantom{\ddag}}$ \cellcolor{green!25} & .0185$^{\phantom{\ddag}}$ \cellcolor{green!18} & .0183$^{\phantom{\ddag}}$ \cellcolor{green!19} & .0175$^{\phantom{\ddag}}$ \cellcolor{green!22} & .0179$^{\phantom{\ddag}}$ \cellcolor{green!21} & .0232$^{\phantom{\ddag}}$ \cellcolor{red!2} & \textbf{.0147}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .0153$^{\phantom{\ddag}}$ \cellcolor{green!32} & .0161$^{\phantom{\ddag}}$ \cellcolor{green!28} \\\cline{2-12}
ctg.2 & .0247$^{\phantom{\ddag}}$ \cellcolor{green!14} & .0332$^{\phantom{\ddag}}$ \cellcolor{red!9} & .0420$^{\phantom{\ddag}}$ \cellcolor{red!35} & .0185$^{\ddag}$ \cellcolor{green!33} & .0186$^{\ddag}$ \cellcolor{green!32} & .0180$^{\ddag}$ \cellcolor{green!34} & .0201$^{\phantom{\ddag}}$ \cellcolor{green!28} & .0192$^{\phantom{\ddag}}$ \cellcolor{green!30} & .0220$^{\phantom{\ddag}}$ \cellcolor{green!22} & \textbf{.0178}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .0193$^{\phantom{\ddag}}$ \cellcolor{green!30} \\\cline{2-12}
ctg.3 & .0260$^{\phantom{\ddag}}$ \cellcolor{green!21} & .0507$^{\phantom{\ddag}}$ \cellcolor{red!19} & .0333$^{\phantom{\ddag}}$ \cellcolor{green!9} & .0381$^{\phantom{\ddag}}$ \cellcolor{green!1} & .0297$^{\phantom{\ddag}}$ \cellcolor{green!15} & .0291$^{\phantom{\ddag}}$ \cellcolor{green!16} & \textbf{.0182}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .0186$^{\ddag}$ \cellcolor{green!34} & .0401$^{\phantom{\ddag}}$ \cellcolor{red!1} & .0597$^{\phantom{\ddag}}$ \cellcolor{red!35} & .0254$^{\phantom{\ddag}}$ \cellcolor{green!22} \\\cline{2-12}
german & .0708$^{\phantom{\ddag}}$ \cellcolor{green!7} & .0591$^{\phantom{\ddag}}$ \cellcolor{green!24} & .0846$^{\phantom{\ddag}}$ \cellcolor{red!11} & .0700$^{\phantom{\ddag}}$ \cellcolor{green!9} & .0700$^{\phantom{\ddag}}$ \cellcolor{green!9} & .0651$^{\phantom{\ddag}}$ \cellcolor{green!15} & .0534$^{\phantom{\ddag}}$ \cellcolor{green!32} & \textbf{.0513}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .0673$^{\phantom{\ddag}}$ \cellcolor{green!12} & .1018$^{\phantom{\ddag}}$ \cellcolor{red!35} & .0838$^{\phantom{\ddag}}$ \cellcolor{red!10} \\\cline{2-12}
haberman & .1523$^{\phantom{\ddag}}$ \cellcolor{green!20} & .1569$^{\phantom{\ddag}}$ \cellcolor{green!19} & .3135$^{\phantom{\ddag}}$ \cellcolor{red!22} & .3010$^{\phantom{\ddag}}$ \cellcolor{red!19} & .3601$^{\phantom{\ddag}}$ \cellcolor{red!35} & \textbf{.0974}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .1214$^{\phantom{\ddag}}$ \cellcolor{green!28} & .1829$^{\phantom{\ddag}}$ \cellcolor{green!12} & .1397$^{\phantom{\ddag}}$ \cellcolor{green!23} & .1355$^{\phantom{\ddag}}$ \cellcolor{green!24} & .1217$^{\phantom{\ddag}}$ \cellcolor{green!28} \\\cline{2-12}
ionosphere & .0671$^{\phantom{\ddag}}$ \cellcolor{red!4} & .0508$^{\phantom{\ddag}}$ \cellcolor{green!15} & .0664$^{\phantom{\ddag}}$ \cellcolor{red!3} & .0373$^{\phantom{\ddag}}$ \cellcolor{green!31} & .0421$^{\phantom{\ddag}}$ \cellcolor{green!25} & \textbf{.0344}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .0923$^{\phantom{\ddag}}$ \cellcolor{red!35} & .0785$^{\phantom{\ddag}}$ \cellcolor{red!18} & .0424$^{\phantom{\ddag}}$ \cellcolor{green!25} & .0347$^{\ddag}$ \cellcolor{green!34} & .0655$^{\phantom{\ddag}}$ \cellcolor{red!2} \\\cline{2-12}
iris.2 & .1622$^{\phantom{\ddag}}$ \cellcolor{red!35} & .0891$^{\phantom{\ddag}}$ \cellcolor{green!1} & .0867$^{\phantom{\ddag}}$ \cellcolor{green!2} & .0251$^{\phantom{\ddag}}$ \cellcolor{green!34} & .0373$^{\phantom{\ddag}}$ \cellcolor{green!27} & .0390$^{\phantom{\ddag}}$ \cellcolor{green!26} & .0384$^{\phantom{\ddag}}$ \cellcolor{green!27} & \textbf{.0231}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .0657$^{\phantom{\ddag}}$ \cellcolor{green!13} & .0980$^{\phantom{\ddag}}$ \cellcolor{red!2} & .0303$^{\phantom{\ddag}}$ \cellcolor{green!31} \\\cline{2-12}
iris.3 & .0678$^{\phantom{\ddag}}$ \cellcolor{red!33} & .0627$^{\phantom{\ddag}}$ \cellcolor{red!26} & \textbf{.0188}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .0678$^{\phantom{\ddag}}$ \cellcolor{red!33} & .0678$^{\phantom{\ddag}}$ \cellcolor{red!33} & .0669$^{\phantom{\ddag}}$ \cellcolor{red!32} & .0678$^{\phantom{\ddag}}$ \cellcolor{red!33} & .0648$^{\phantom{\ddag}}$ \cellcolor{red!29} & .0676$^{\phantom{\ddag}}$ \cellcolor{red!33} & .0628$^{\phantom{\ddag}}$ \cellcolor{red!26} & .0687$^{\phantom{\ddag}}$ \cellcolor{red!35} \\\cline{2-12}
mammographic & .0497$^{\phantom{\ddag}}$ \cellcolor{green!7} & .0432$^{\phantom{\ddag}}$ \cellcolor{green!23} & .0664$^{\phantom{\ddag}}$ \cellcolor{red!34} & .0424$^{\phantom{\ddag}}$ \cellcolor{green!25} & .0426$^{\phantom{\ddag}}$ \cellcolor{green!25} & .0438$^{\phantom{\ddag}}$ \cellcolor{green!22} & \textbf{.0388}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .0465$^{\phantom{\ddag}}$ \cellcolor{green!15} & .0664$^{\phantom{\ddag}}$ \cellcolor{red!35} & .0425$^{\phantom{\ddag}}$ \cellcolor{green!25} & .0400$^{\dag}$ \cellcolor{green!31} \\\cline{2-12}
pageblocks.5 & .0286$^{\phantom{\ddag}}$ \cellcolor{green!32} & .0221$^{\phantom{\ddag}}$ \cellcolor{green!33} & .0953$^{\phantom{\ddag}}$ \cellcolor{green!17} & .0223$^{\phantom{\ddag}}$ \cellcolor{green!33} & .0206$^{\phantom{\ddag}}$ \cellcolor{green!34} & .0195$^{\phantom{\ddag}}$ \cellcolor{green!34} & .0228$^{\phantom{\ddag}}$ \cellcolor{green!33} & .0205$^{\phantom{\ddag}}$ \cellcolor{green!34} & .3395$^{\phantom{\ddag}}$ \cellcolor{red!35} & \textbf{.0167}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .0189$^{\phantom{\ddag}}$ \cellcolor{green!34} \\\cline{2-12}
semeion & .0223$^{\phantom{\ddag}}$ \cellcolor{red!3} & .0308$^{\phantom{\ddag}}$ \cellcolor{red!35} & .0242$^{\phantom{\ddag}}$ \cellcolor{red!10} & .0170$^{\phantom{\ddag}}$ \cellcolor{green!16} & .0199$^{\phantom{\ddag}}$ \cellcolor{green!6} & .0150$^{\phantom{\ddag}}$ \cellcolor{green!24} & .0176$^{\phantom{\ddag}}$ \cellcolor{green!14} & .0179$^{\phantom{\ddag}}$ \cellcolor{green!13} & .0281$^{\phantom{\ddag}}$ \cellcolor{red!24} & \textbf{.0122}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .0180$^{\phantom{\ddag}}$ \cellcolor{green!13} \\\cline{2-12}
sonar & .1636$^{\phantom{\ddag}}$ \cellcolor{red!35} & .1553$^{\phantom{\ddag}}$ \cellcolor{red!29} & .1317$^{\phantom{\ddag}}$ \cellcolor{red!15} & .0660$^{\phantom{\ddag}}$ \cellcolor{green!25} & .0687$^{\phantom{\ddag}}$ \cellcolor{green!23} & \textbf{.0499}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .0618$^{\phantom{\ddag}}$ \cellcolor{green!27} & .0525$^{\dag}$ \cellcolor{green!33} & .0999$^{\phantom{\ddag}}$ \cellcolor{green!4} & .0673$^{\phantom{\ddag}}$ \cellcolor{green!24} & .0586$^{\phantom{\ddag}}$ \cellcolor{green!29} \\\cline{2-12}
spambase & .0230$^{\phantom{\ddag}}$ \cellcolor{green!22} & .0206$^{\phantom{\ddag}}$ \cellcolor{green!29} & .0236$^{\phantom{\ddag}}$ \cellcolor{green!21} & .0189$^{\dag}$ \cellcolor{green!33} & .0191$^{\dag}$ \cellcolor{green!33} & .0187$^{\ddag}$ \cellcolor{green!34} & .0203$^{\phantom{\ddag}}$ \cellcolor{green!29} & .0195$^{\phantom{\ddag}}$ \cellcolor{green!32} & .0448$^{\phantom{\ddag}}$ \cellcolor{red!35} & .0195$^{\phantom{\ddag}}$ \cellcolor{green!32} & \textbf{.0184}$^{\phantom{\ddag}}$ \cellcolor{green!35} \\\cline{2-12}
spectf & .1996$^{\phantom{\ddag}}$ \cellcolor{red!35} & .0508$^{\phantom{\ddag}}$ \cellcolor{green!28} & .1888$^{\phantom{\ddag}}$ \cellcolor{red!30} & .0410$^{\phantom{\ddag}}$ \cellcolor{green!32} & .0409$^{\phantom{\ddag}}$ \cellcolor{green!32} & \textbf{.0362}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .0441$^{\phantom{\ddag}}$ \cellcolor{green!31} & .0433$^{\phantom{\ddag}}$ \cellcolor{green!31} & .0638$^{\phantom{\ddag}}$ \cellcolor{green!23} & .1205$^{\phantom{\ddag}}$ \cellcolor{red!1} & .0439$^{\phantom{\ddag}}$ \cellcolor{green!31} \\\cline{2-12}
tictactoe & .0095$^{\phantom{\ddag}}$ \cellcolor{green!18} & .0090$^{\phantom{\ddag}}$ \cellcolor{green!22} & .0098$^{\phantom{\ddag}}$ \cellcolor{green!16} & .0083$^{\phantom{\ddag}}$ \cellcolor{green!27} & .0078$^{\phantom{\ddag}}$ \cellcolor{green!32} & .0083$^{\phantom{\ddag}}$ \cellcolor{green!28} & \textbf{.0074}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .0076$^{\ddag}$ \cellcolor{green!33} & .0164$^{\phantom{\ddag}}$ \cellcolor{red!35} & .0075$^{\ddag}$ \cellcolor{green!34} & .0109$^{\phantom{\ddag}}$ \cellcolor{green!7} \\\cline{2-12}
transfusion & .1036$^{\phantom{\ddag}}$ \cellcolor{green!16} & .0817$^{\phantom{\ddag}}$ \cellcolor{green!27} & .2086$^{\phantom{\ddag}}$ \cellcolor{red!35} & .0738$^{\phantom{\ddag}}$ \cellcolor{green!31} & .0738$^{\phantom{\ddag}}$ \cellcolor{green!31} & \textbf{.0660}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .0761$^{\phantom{\ddag}}$ \cellcolor{green!30} & .0733$^{\phantom{\ddag}}$ \cellcolor{green!31} & .0959$^{\phantom{\ddag}}$ \cellcolor{green!20} & .0678$^{\phantom{\ddag}}$ \cellcolor{green!34} & .0719$^{\phantom{\ddag}}$ \cellcolor{green!32} \\\cline{2-12}
wdbc & .0200$^{\phantom{\ddag}}$ \cellcolor{green!9} & .0169$^{\phantom{\ddag}}$ \cellcolor{green!17} & .0358$^{\phantom{\ddag}}$ \cellcolor{red!35} & \textbf{.0108}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .0121$^{\phantom{\ddag}}$ \cellcolor{green!31} & .0136$^{\phantom{\ddag}}$ \cellcolor{green!26} & .0162$^{\phantom{\ddag}}$ \cellcolor{green!19} & .0188$^{\phantom{\ddag}}$ \cellcolor{green!12} & .0208$^{\phantom{\ddag}}$ \cellcolor{green!6} & .0130$^{\phantom{\ddag}}$ \cellcolor{green!28} & .0190$^{\phantom{\ddag}}$ \cellcolor{green!11} \\\cline{2-12}
wine.1 & .0301$^{\phantom{\ddag}}$ \cellcolor{green!19} & .0378$^{\phantom{\ddag}}$ \cellcolor{green!13} & .1045$^{\phantom{\ddag}}$ \cellcolor{red!35} & .0219$^{\phantom{\ddag}}$ \cellcolor{green!25} & \textbf{.0085}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .0133$^{\phantom{\ddag}}$ \cellcolor{green!31} & .0222$^{\phantom{\ddag}}$ \cellcolor{green!25} & .0212$^{\phantom{\ddag}}$ \cellcolor{green!25} & .0221$^{\phantom{\ddag}}$ \cellcolor{green!25} & .0130$^{\phantom{\ddag}}$ \cellcolor{green!31} & .0096$^{\phantom{\ddag}}$ \cellcolor{green!34} \\\cline{2-12}
wine.2 & .0273$^{\phantom{\ddag}}$ \cellcolor{red!35} & .0242$^{\phantom{\ddag}}$ \cellcolor{red!23} & .0198$^{\phantom{\ddag}}$ \cellcolor{red!7} & .0108$^{\phantom{\ddag}}$ \cellcolor{green!25} & .0109$^{\phantom{\ddag}}$ \cellcolor{green!25} & .0114$^{\phantom{\ddag}}$ \cellcolor{green!23} & .0120$^{\phantom{\ddag}}$ \cellcolor{green!21} & .0115$^{\phantom{\ddag}}$ \cellcolor{green!23} & .0128$^{\phantom{\ddag}}$ \cellcolor{green!18} & .0094$^{\phantom{\ddag}}$ \cellcolor{green!31} & \textbf{.0083}$^{\phantom{\ddag}}$ \cellcolor{green!35} \\\cline{2-12}
wine.3 & .0524$^{\phantom{\ddag}}$ \cellcolor{red!35} & .0300$^{\phantom{\ddag}}$ \cellcolor{green!2} & .0385$^{\phantom{\ddag}}$ \cellcolor{red!11} & .0144$^{\phantom{\ddag}}$ \cellcolor{green!28} & .0176$^{\phantom{\ddag}}$ \cellcolor{green!22} & .0128$^{\phantom{\ddag}}$ \cellcolor{green!31} & .0242$^{\phantom{\ddag}}$ \cellcolor{green!11} & .0234$^{\phantom{\ddag}}$ \cellcolor{green!13} & .0392$^{\phantom{\ddag}}$ \cellcolor{red!13} & .0173$^{\phantom{\ddag}}$ \cellcolor{green!23} & \textbf{.0104}$^{\phantom{\ddag}}$ \cellcolor{green!35} \\\cline{2-12}
wine-q-red & .0597$^{\phantom{\ddag}}$ \cellcolor{red!35} & .0497$^{\ddag}$ \cellcolor{green!23} & .0526$^{\phantom{\ddag}}$ \cellcolor{green!6} & .0494$^{\phantom{\ddag}}$ \cellcolor{green!25} & .0496$^{\phantom{\ddag}}$ \cellcolor{green!24} & .0593$^{\phantom{\ddag}}$ \cellcolor{red!32} & .0560$^{\phantom{\ddag}}$ \cellcolor{red!13} & .0543$^{\phantom{\ddag}}$ \cellcolor{red!3} & .0487$^{\ddag}$ \cellcolor{green!29} & .0478$^{\ddag}$ \cellcolor{green!34} & \textbf{.0478}$^{\phantom{\ddag}}$ \cellcolor{green!35} \\\cline{2-12}
wine-q-white & .0986$^{\phantom{\ddag}}$ \cellcolor{red!35} & .0675$^{\phantom{\ddag}}$ \cellcolor{green!28} & .0764$^{\phantom{\ddag}}$ \cellcolor{green!9} & .0703$^{\phantom{\ddag}}$ \cellcolor{green!22} & .0669$^{\phantom{\ddag}}$ \cellcolor{green!29} & .0694$^{\phantom{\ddag}}$ \cellcolor{green!24} & .0703$^{\phantom{\ddag}}$ \cellcolor{green!22} & .0740$^{\phantom{\ddag}}$ \cellcolor{green!14} & .0649$^{\dag}$ \cellcolor{green!33} & \textbf{.0641}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .0656$^{\phantom{\ddag}}$ \cellcolor{green!31} \\\cline{2-12}
yeast & .1262$^{\phantom{\ddag}}$ \cellcolor{red!35} & .1052$^{\phantom{\ddag}}$ \cellcolor{red!11} & .0679$^{\dag}$ \cellcolor{green!29} & .0715$^{\phantom{\ddag}}$ \cellcolor{green!25} & .0708$^{\phantom{\ddag}}$ \cellcolor{green!25} & \textbf{.0626}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .0809$^{\phantom{\ddag}}$ \cellcolor{green!14} & .0753$^{\phantom{\ddag}}$ \cellcolor{green!20} & .0842$^{\phantom{\ddag}}$ \cellcolor{green!11} & .0995$^{\phantom{\ddag}}$ \cellcolor{red!5} & .0776$^{\phantom{\ddag}}$ \cellcolor{green!18} \\\cline{2-12}
\hline 
 \textit{\textit{Average}} & .0696$^{\phantom{\ddag}}$ \cellcolor{red!11} & .0568$^{\phantom{\ddag}}$ \cellcolor{green!10} & .0834$^{\phantom{\ddag}}$ \cellcolor{red!35} & .0543$^{\phantom{\ddag}}$ \cellcolor{green!14} & .0565$^{\phantom{\ddag}}$ \cellcolor{green!11} & \textbf{.0425}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .0491$^{\phantom{\ddag}}$ \cellcolor{green!23} & .0496$^{\phantom{\ddag}}$ \cellcolor{green!22} & .0619$^{\phantom{\ddag}}$ \cellcolor{green!1} & .0512$^{\phantom{\ddag}}$ \cellcolor{green!20} & .0453$^{\phantom{\ddag}}$ \cellcolor{green!30} \\\cline{2-12}
\textit{Rank} &  8.8 \cellcolor{red!35} &  7.0 \cellcolor{red!8} &  8.3 \cellcolor{red!27} &  5.2 \cellcolor{green!17} &  5.3 \cellcolor{green!17} & \textbf{4.1} \cellcolor{green!35} &  6.1 \cellcolor{green!4} &  5.8 \cellcolor{green!9} &  6.3 \cellcolor{green!1} &  4.4 \cellcolor{green!29} &  4.6 \cellcolor{green!27} \\\hline

\end{tabular}

==> tables/tab_uci_mrae.tex <==

            \begin{tabular}{|c|c|c|c|c||c|c||c|c||c|c|c|} \cline{2-12}
            \multicolumn{1}{c}{} & 
            \multicolumn{2}{|c}{Adjustment} & 
            \multicolumn{6}{|c|}{Distribution Matching} & 
            \multicolumn{3}{c|}{Maximum Likelihood} \\
             \cline{2-12} 
            \multicolumn{1}{c|}{} & ACC & PACC & HDy & DM-T & DM-HD & KDEy-HD & DM-CS & KDEy-CS & DIR & EMQ & KDEy-ML \\\hline
balance.1 &  0.0711$^{\dag}$ \cellcolor{green!21} &  0.0539$^{\phantom{\ddag}}$ \cellcolor{green!32} &  0.0679$^{\phantom{\ddag}}$ \cellcolor{green!23} & \textbf{0.0507}$^{\phantom{\ddag}}$ \cellcolor{green!35} &  0.0779$^{\phantom{\ddag}}$ \cellcolor{green!17} &  0.0746$^{\phantom{\ddag}}$ \cellcolor{green!19} &  0.1576$^{\phantom{\ddag}}$ \cellcolor{red!35} &  0.1496$^{\phantom{\ddag}}$ \cellcolor{red!29} &  0.0603$^{\dag}$ \cellcolor{green!28} &  0.0676$^{\phantom{\ddag}}$ \cellcolor{green!23} &  0.0953$^{\phantom{\ddag}}$ \cellcolor{green!5} \\\cline{2-12}
balance.3 &  0.1197$^{\phantom{\ddag}}$ \cellcolor{red!13} &  0.1150$^{\phantom{\ddag}}$ \cellcolor{red!9} &  0.1262$^{\phantom{\ddag}}$ \cellcolor{red!19} &  0.0906$^{\phantom{\ddag}}$ \cellcolor{green!11} &  0.1113$^{\phantom{\ddag}}$ \cellcolor{red!6} &  0.1059$^{\phantom{\ddag}}$ \cellcolor{red!1} &  0.1439$^{\phantom{\ddag}}$ \cellcolor{red!35} &  0.1284$^{\phantom{\ddag}}$ \cellcolor{red!21} & \textbf{0.0636}$^{\phantom{\ddag}}$ \cellcolor{green!35} &  0.1072$^{\phantom{\ddag}}$ \cellcolor{red!3} &  0.1113$^{\phantom{\ddag}}$ \cellcolor{red!6} \\\cline{2-12}
breast-cancer &  0.1242$^{\phantom{\ddag}}$ \cellcolor{red!27} &  0.1148$^{\phantom{\ddag}}$ \cellcolor{red!21} &  0.1341$^{\phantom{\ddag}}$ \cellcolor{red!35} &  0.0754$^{\phantom{\ddag}}$ \cellcolor{green!7} &  0.0919$^{\phantom{\ddag}}$ \cellcolor{red!4} &  0.0724$^{\phantom{\ddag}}$ \cellcolor{green!9} &  0.0496$^{\phantom{\ddag}}$ \cellcolor{green!25} &  0.0425$^{\phantom{\ddag}}$ \cellcolor{green!30} &  0.0694$^{\phantom{\ddag}}$ \cellcolor{green!11} & \textbf{0.0366}$^{\phantom{\ddag}}$ \cellcolor{green!35} &  0.0383$^{\phantom{\ddag}}$ \cellcolor{green!33} \\\cline{2-12}
cmc.1 &  0.6474$^{\phantom{\ddag}}$ \cellcolor{red!35} &  0.4079$^{\phantom{\ddag}}$ \cellcolor{green!17} &  0.5414$^{\dag}$ \cellcolor{red!11} &  0.3389$^{\phantom{\ddag}}$ \cellcolor{green!32} &  0.3491$^{\phantom{\ddag}}$ \cellcolor{green!30} & \textbf{0.3266}$^{\phantom{\ddag}}$ \cellcolor{green!35} &  0.4761$^{\phantom{\ddag}}$ \cellcolor{green!2} &  0.3795$^{\phantom{\ddag}}$ \cellcolor{green!23} &  0.4721$^{\dag}$ \cellcolor{green!3} &  0.3477$^{\phantom{\ddag}}$ \cellcolor{green!30} &  0.3304$^{\phantom{\ddag}}$ \cellcolor{green!34} \\\cline{2-12}
cmc.2 &  0.4931$^{\phantom{\ddag}}$ \cellcolor{green!22} &  0.4446$^{\phantom{\ddag}}$ \cellcolor{green!25} &  1.4550$^{\phantom{\ddag}}$ \cellcolor{red!35} &  0.7913$^{\phantom{\ddag}}$ \cellcolor{green!4} &  0.7855$^{\phantom{\ddag}}$ \cellcolor{green!4} &  0.3568$^{\phantom{\ddag}}$ \cellcolor{green!30} &  0.6900$^{\phantom{\ddag}}$ \cellcolor{green!10} &  0.5860$^{\phantom{\ddag}}$ \cellcolor{green!16} & \textbf{0.2804}$^{\phantom{\ddag}}$ \cellcolor{green!35} &  0.3044$^{\phantom{\ddag}}$ \cellcolor{green!33} &  0.3139$^{\phantom{\ddag}}$ \cellcolor{green!33} \\\cline{2-12}
cmc.3 &  0.5405$^{\phantom{\ddag}}$ \cellcolor{red!1} &  0.6774$^{\phantom{\ddag}}$ \cellcolor{red!35} &  0.6231$^{\ddag}$ \cellcolor{red!21} &  0.4385$^{\ddag}$ \cellcolor{green!23} &  0.4238$^{\ddag}$ \cellcolor{green!27} &  0.4105$^{\phantom{\ddag}}$ \cellcolor{green!30} &  0.5258$^{\phantom{\ddag}}$ \cellcolor{green!2} &  0.4884$^{\phantom{\ddag}}$ \cellcolor{green!11} &  0.6139$^{\dag}$ \cellcolor{red!19} &  0.4160$^{\ddag}$ \cellcolor{green!29} & \textbf{0.3933}$^{\phantom{\ddag}}$ \cellcolor{green!35} \\\cline{2-12}
ctg.1 &  0.0790$^{\phantom{\ddag}}$ \cellcolor{red!8} &  0.0907$^{\phantom{\ddag}}$ \cellcolor{red!35} &  0.0791$^{\phantom{\ddag}}$ \cellcolor{red!8} &  0.0692$^{\phantom{\ddag}}$ \cellcolor{green!14} &  0.0686$^{\phantom{\ddag}}$ \cellcolor{green!15} &  0.0659$^{\phantom{\ddag}}$ \cellcolor{green!21} &  0.0805$^{\phantom{\ddag}}$ \cellcolor{red!11} &  0.0782$^{\phantom{\ddag}}$ \cellcolor{red!6} &  0.0824$^{\phantom{\ddag}}$ \cellcolor{red!16} & \textbf{0.0600}$^{\phantom{\ddag}}$ \cellcolor{green!35} &  0.0627$^{\ddag}$ \cellcolor{green!28} \\\cline{2-12}
ctg.2 &  0.1208$^{\phantom{\ddag}}$ \cellcolor{green!8} &  0.1725$^{\phantom{\ddag}}$ \cellcolor{red!31} &  0.1765$^{\phantom{\ddag}}$ \cellcolor{red!35} &  0.0951$^{\ddag}$ \cellcolor{green!28} &  0.0957$^{\ddag}$ \cellcolor{green!28} &  0.0899$^{\ddag}$ \cellcolor{green!32} &  0.0954$^{\phantom{\ddag}}$ \cellcolor{green!28} &  0.0970$^{\dag}$ \cellcolor{green!27} &  0.1228$^{\phantom{\ddag}}$ \cellcolor{green!6} & \textbf{0.0868}$^{\phantom{\ddag}}$ \cellcolor{green!35} &  0.0980$^{\ddag}$ \cellcolor{green!26} \\\cline{2-12}
ctg.3 &  0.1363$^{\phantom{\ddag}}$ \cellcolor{green!5} &  0.2331$^{\phantom{\ddag}}$ \cellcolor{red!35} &  0.1194$^{\phantom{\ddag}}$ \cellcolor{green!12} &  0.1235$^{\phantom{\ddag}}$ \cellcolor{green!11} &  0.1810$^{\phantom{\ddag}}$ \cellcolor{red!13} &  0.1267$^{\phantom{\ddag}}$ \cellcolor{green!9} &  0.0713$^{\phantom{\ddag}}$ \cellcolor{green!33} & \textbf{0.0669}$^{\phantom{\ddag}}$ \cellcolor{green!35} &  0.1731$^{\phantom{\ddag}}$ \cellcolor{red!9} &  0.0729$^{\ddag}$ \cellcolor{green!32} &  0.0996$^{\phantom{\ddag}}$ \cellcolor{green!21} \\\cline{2-12}
german &  0.4036$^{\phantom{\ddag}}$ \cellcolor{green!11} &  0.3047$^{\phantom{\ddag}}$ \cellcolor{green!23} &  0.7942$^{\phantom{\ddag}}$ \cellcolor{red!35} &  0.2269$^{\phantom{\ddag}}$ \cellcolor{green!32} &  0.4666$^{\phantom{\ddag}}$ \cellcolor{green!4} &  0.2392$^{\phantom{\ddag}}$ \cellcolor{green!31} &  0.2129$^{\phantom{\ddag}}$ \cellcolor{green!34} & \textbf{0.2097}$^{\phantom{\ddag}}$ \cellcolor{green!35} &  0.2391$^{\phantom{\ddag}}$ \cellcolor{green!31} &  0.3378$^{\phantom{\ddag}}$ \cellcolor{green!19} &  0.3022$^{\phantom{\ddag}}$ \cellcolor{green!23} \\\cline{2-12}
haberman &  1.0928$^{\phantom{\ddag}}$ \cellcolor{green!1} &  0.5040$^{\phantom{\ddag}}$ \cellcolor{green!29} &  1.4905$^{\phantom{\ddag}}$ \cellcolor{red!17} &  1.5918$^{\phantom{\ddag}}$ \cellcolor{red!21} &  1.8737$^{\phantom{\ddag}}$ \cellcolor{red!35} & \textbf{0.3830}$^{\phantom{\ddag}}$ \cellcolor{green!35} &  1.1789$^{\phantom{\ddag}}$ \cellcolor{red!2} &  1.1870$^{\phantom{\ddag}}$ \cellcolor{red!2} &  0.4995$^{\phantom{\ddag}}$ \cellcolor{green!29} &  0.4095$^{\phantom{\ddag}}$ \cellcolor{green!33} &  0.4165$^{\phantom{\ddag}}$ \cellcolor{green!33} \\\cline{2-12}
ionosphere &  0.3416$^{\phantom{\ddag}}$ \cellcolor{red!4} &  0.2401$^{\phantom{\ddag}}$ \cellcolor{green!15} &  0.2735$^{\phantom{\ddag}}$ \cellcolor{green!8} & \textbf{0.1377}$^{\phantom{\ddag}}$ \cellcolor{green!35} &  0.1499$^{\phantom{\ddag}}$ \cellcolor{green!32} &  0.1429$^{\phantom{\ddag}}$ \cellcolor{green!34} &  0.4983$^{\phantom{\ddag}}$ \cellcolor{red!35} &  0.4145$^{\phantom{\ddag}}$ \cellcolor{red!18} &  0.3426$^{\phantom{\ddag}}$ \cellcolor{red!4} &  0.1847$^{\ddag}$ \cellcolor{green!25} &  0.3691$^{\phantom{\ddag}}$ \cellcolor{red!9} \\\cline{2-12}
iris.2 &  0.4885$^{\phantom{\ddag}}$ \cellcolor{red!16} &  0.3253$^{\phantom{\ddag}}$ \cellcolor{green!5} &  0.2914$^{\phantom{\ddag}}$ \cellcolor{green!10} &  0.1737$^{\phantom{\ddag}}$ \cellcolor{green!26} &  0.1383$^{\phantom{\ddag}}$ \cellcolor{green!31} &  0.1260$^{\phantom{\ddag}}$ \cellcolor{green!32} &  0.1801$^{\phantom{\ddag}}$ \cellcolor{green!25} &  0.1250$^{\phantom{\ddag}}$ \cellcolor{green!33} &  0.6283$^{\phantom{\ddag}}$ \cellcolor{red!35} &  0.4765$^{\phantom{\ddag}}$ \cellcolor{red!14} & \textbf{0.1104}$^{\phantom{\ddag}}$ \cellcolor{green!35} \\\cline{2-12}
iris.3 &  0.3793$^{\phantom{\ddag}}$ \cellcolor{red!31} &  0.3328$^{\phantom{\ddag}}$ \cellcolor{red!19} & \textbf{0.1124}$^{\phantom{\ddag}}$ \cellcolor{green!35} &  0.3797$^{\phantom{\ddag}}$ \cellcolor{red!31} &  0.3793$^{\phantom{\ddag}}$ \cellcolor{red!31} &  0.3695$^{\phantom{\ddag}}$ \cellcolor{red!28} &  0.3795$^{\phantom{\ddag}}$ \cellcolor{red!31} &  0.3622$^{\phantom{\ddag}}$ \cellcolor{red!27} &  0.3802$^{\phantom{\ddag}}$ \cellcolor{red!31} &  0.3305$^{\phantom{\ddag}}$ \cellcolor{red!19} &  0.3941$^{\phantom{\ddag}}$ \cellcolor{red!35} \\\cline{2-12}
mammographic &  0.3207$^{\phantom{\ddag}}$ \cellcolor{green!4} &  0.2902$^{\phantom{\ddag}}$ \cellcolor{green!10} &  0.4718$^{\phantom{\ddag}}$ \cellcolor{red!27} &  0.2384$^{\phantom{\ddag}}$ \cellcolor{green!21} &  0.2373$^{\phantom{\ddag}}$ \cellcolor{green!21} &  0.2506$^{\phantom{\ddag}}$ \cellcolor{green!18} &  0.2518$^{\phantom{\ddag}}$ \cellcolor{green!18} &  0.2624$^{\phantom{\ddag}}$ \cellcolor{green!16} &  0.5055$^{\phantom{\ddag}}$ \cellcolor{red!35} & \textbf{0.1742}$^{\phantom{\ddag}}$ \cellcolor{green!35} &  0.1795$^{\phantom{\ddag}}$ \cellcolor{green!33} \\\cline{2-12}
pageblocks.5 &  0.1399$^{\phantom{\ddag}}$ \cellcolor{green!32} &  0.1117$^{\phantom{\ddag}}$ \cellcolor{green!34} &  0.3137$^{\phantom{\ddag}}$ \cellcolor{green!26} &  0.0961$^{\phantom{\ddag}}$ \cellcolor{green!34} &  0.0886$^{\ddag}$ \cellcolor{green!34} & \textbf{0.0870}$^{\phantom{\ddag}}$ \cellcolor{green!35} &  0.0894$^{\dag}$ \cellcolor{green!34} &  0.0871$^{\ddag}$ \cellcolor{green!34} &  1.8883$^{\phantom{\ddag}}$ \cellcolor{red!35} &  0.0962$^{\phantom{\ddag}}$ \cellcolor{green!34} &  0.0914$^{\phantom{\ddag}}$ \cellcolor{green!34} \\\cline{2-12}
semeion &  0.2790$^{\phantom{\ddag}}$ \cellcolor{red!35} &  0.1729$^{\phantom{\ddag}}$ \cellcolor{red!3} &  0.0875$^{\phantom{\ddag}}$ \cellcolor{green!22} &  0.1603$^{\phantom{\ddag}}$ \cellcolor{green!0} &  0.1868$^{\phantom{\ddag}}$ \cellcolor{red!7} &  0.0631$^{\phantom{\ddag}}$ \cellcolor{green!29} &  0.0764$^{\phantom{\ddag}}$ \cellcolor{green!25} &  0.0676$^{\phantom{\ddag}}$ \cellcolor{green!28} &  0.0745$^{\phantom{\ddag}}$ \cellcolor{green!26} & \textbf{0.0458}$^{\phantom{\ddag}}$ \cellcolor{green!35} &  0.0694$^{\phantom{\ddag}}$ \cellcolor{green!27} \\\cline{2-12}
sonar &  0.8184$^{\phantom{\ddag}}$ \cellcolor{red!35} &  0.5921$^{\phantom{\ddag}}$ \cellcolor{red!10} &  0.7457$^{\phantom{\ddag}}$ \cellcolor{red!27} &  0.2212$^{\phantom{\ddag}}$ \cellcolor{green!29} &  0.2278$^{\phantom{\ddag}}$ \cellcolor{green!29} & \textbf{0.1729}$^{\phantom{\ddag}}$ \cellcolor{green!35} &  0.2283$^{\phantom{\ddag}}$ \cellcolor{green!28} &  0.2135$^{\phantom{\ddag}}$ \cellcolor{green!30} &  0.5266$^{\phantom{\ddag}}$ \cellcolor{red!3} &  0.3445$^{\phantom{\ddag}}$ \cellcolor{green!16} &  0.1949$^{\phantom{\ddag}}$ \cellcolor{green!32} \\\cline{2-12}
spambase &  0.1115$^{\phantom{\ddag}}$ \cellcolor{green!26} &  0.0959$^{\phantom{\ddag}}$ \cellcolor{green!31} &  0.0979$^{\phantom{\ddag}}$ \cellcolor{green!30} & \textbf{0.0821}$^{\phantom{\ddag}}$ \cellcolor{green!35} &  0.0822$^{\ddag}$ \cellcolor{green!34} &  0.0825$^{\ddag}$ \cellcolor{green!34} &  0.0895$^{\phantom{\ddag}}$ \cellcolor{green!32} &  0.0856$^{\phantom{\ddag}}$ \cellcolor{green!33} &  0.3316$^{\phantom{\ddag}}$ \cellcolor{red!35} &  0.0933$^{\dag}$ \cellcolor{green!31} &  0.0830$^{\ddag}$ \cellcolor{green!34} \\\cline{2-12}
spectf &  0.5731$^{\phantom{\ddag}}$ \cellcolor{green!1} &  0.3352$^{\phantom{\ddag}}$ \cellcolor{green!20} &  1.0476$^{\phantom{\ddag}}$ \cellcolor{red!35} &  0.1808$^{\phantom{\ddag}}$ \cellcolor{green!32} &  0.1962$^{\phantom{\ddag}}$ \cellcolor{green!31} & \textbf{0.1460}$^{\phantom{\ddag}}$ \cellcolor{green!35} &  0.1812$^{\phantom{\ddag}}$ \cellcolor{green!32} &  0.1745$^{\phantom{\ddag}}$ \cellcolor{green!32} &  0.3253$^{\phantom{\ddag}}$ \cellcolor{green!21} &  0.1528$^{\phantom{\ddag}}$ \cellcolor{green!34} &  0.1636$^{\phantom{\ddag}}$ \cellcolor{green!33} \\\cline{2-12}
tictactoe &  0.0413$^{\ddag}$ \cellcolor{green!25} &  0.0391$^{\dag}$ \cellcolor{green!27} & \textbf{0.0309}$^{\phantom{\ddag}}$ \cellcolor{green!35} &  0.0360$^{\phantom{\ddag}}$ \cellcolor{green!30} &  0.0419$^{\ddag}$ \cellcolor{green!24} &  0.0326$^{\phantom{\ddag}}$ \cellcolor{green!33} &  0.0326$^{\phantom{\ddag}}$ \cellcolor{green!33} &  0.0314$^{\phantom{\ddag}}$ \cellcolor{green!34} &  0.1057$^{\phantom{\ddag}}$ \cellcolor{red!35} &  0.0309$^{\phantom{\ddag}}$ \cellcolor{green!34} &  0.0360$^{\phantom{\ddag}}$ \cellcolor{green!30} \\\cline{2-12}
transfusion &  0.5497$^{\phantom{\ddag}}$ \cellcolor{green!13} &  0.4059$^{\phantom{\ddag}}$ \cellcolor{green!24} &  1.1953$^{\phantom{\ddag}}$ \cellcolor{red!35} &  0.2879$^{\ddag}$ \cellcolor{green!32} &  0.2877$^{\ddag}$ \cellcolor{green!33} &  0.2948$^{\phantom{\ddag}}$ \cellcolor{green!32} &  0.3265$^{\phantom{\ddag}}$ \cellcolor{green!30} &  0.3837$^{\ddag}$ \cellcolor{green!25} &  0.4142$^{\phantom{\ddag}}$ \cellcolor{green!23} & \textbf{0.2610}$^{\phantom{\ddag}}$ \cellcolor{green!35} &  0.3388$^{\phantom{\ddag}}$ \cellcolor{green!29} \\\cline{2-12}
wdbc &  0.0901$^{\phantom{\ddag}}$ \cellcolor{green!8} &  0.1105$^{\phantom{\ddag}}$ \cellcolor{red!4} &  0.0723$^{\phantom{\ddag}}$ \cellcolor{green!20} &  0.0507$^{\dag}$ \cellcolor{green!34} & \textbf{0.0503}$^{\phantom{\ddag}}$ \cellcolor{green!35} &  0.0800$^{\phantom{\ddag}}$ \cellcolor{green!15} &  0.0626$^{\phantom{\ddag}}$ \cellcolor{green!26} &  0.0636$^{\phantom{\ddag}}$ \cellcolor{green!26} &  0.1560$^{\phantom{\ddag}}$ \cellcolor{red!35} &  0.0633$^{\phantom{\ddag}}$ \cellcolor{green!26} &  0.0809$^{\phantom{\ddag}}$ \cellcolor{green!14} \\\cline{2-12}
wine.1 &  0.1873$^{\phantom{\ddag}}$ \cellcolor{red!2} &  0.1676$^{\phantom{\ddag}}$ \cellcolor{green!2} &  0.3064$^{\phantom{\ddag}}$ \cellcolor{red!35} &  0.1004$^{\phantom{\ddag}}$ \cellcolor{green!20} &  0.1171$^{\phantom{\ddag}}$ \cellcolor{green!16} &  0.0619$^{\phantom{\ddag}}$ \cellcolor{green!31} &  0.0992$^{\phantom{\ddag}}$ \cellcolor{green!21} &  0.1012$^{\phantom{\ddag}}$ \cellcolor{green!20} &  0.0935$^{\phantom{\ddag}}$ \cellcolor{green!22} &  0.0504$^{\phantom{\ddag}}$ \cellcolor{green!34} & \textbf{0.0483}$^{\phantom{\ddag}}$ \cellcolor{green!35} \\\cline{2-12}
wine.2 &  0.1155$^{\phantom{\ddag}}$ \cellcolor{red!35} &  0.1055$^{\phantom{\ddag}}$ \cellcolor{red!26} &  0.0745$^{\phantom{\ddag}}$ \cellcolor{red!0} &  0.0463$^{\phantom{\ddag}}$ \cellcolor{green!23} &  0.0549$^{\phantom{\ddag}}$ \cellcolor{green!15} &  0.0402$^{\phantom{\ddag}}$ \cellcolor{green!28} &  0.0555$^{\phantom{\ddag}}$ \cellcolor{green!15} &  0.0369$^{\phantom{\ddag}}$ \cellcolor{green!30} &  0.0624$^{\phantom{\ddag}}$ \cellcolor{green!9} &  0.0326$^{\dag}$ \cellcolor{green!34} & \textbf{0.0320}$^{\phantom{\ddag}}$ \cellcolor{green!35} \\\cline{2-12}
wine.3 &  0.2123$^{\phantom{\ddag}}$ \cellcolor{red!35} &  0.1218$^{\phantom{\ddag}}$ \cellcolor{green!4} &  0.1300$^{\phantom{\ddag}}$ \cellcolor{green!0} &  0.0695$^{\phantom{\ddag}}$ \cellcolor{green!27} &  0.0673$^{\phantom{\ddag}}$ \cellcolor{green!28} &  0.1229$^{\phantom{\ddag}}$ \cellcolor{green!3} &  0.0735$^{\phantom{\ddag}}$ \cellcolor{green!25} &  0.0820$^{\phantom{\ddag}}$ \cellcolor{green!21} &  0.1497$^{\phantom{\ddag}}$ \cellcolor{red!7} &  0.0555$^{\phantom{\ddag}}$ \cellcolor{green!33} & \textbf{0.0517}$^{\phantom{\ddag}}$ \cellcolor{green!35} \\\cline{2-12}
wine-q-red &  0.2698$^{\phantom{\ddag}}$ \cellcolor{red!35} &  0.2269$^{\phantom{\ddag}}$ \cellcolor{green!9} &  0.2593$^{\ddag}$ \cellcolor{red!24} &  0.2142$^{\phantom{\ddag}}$ \cellcolor{green!22} &  0.2141$^{\phantom{\ddag}}$ \cellcolor{green!22} &  0.2172$^{\phantom{\ddag}}$ \cellcolor{green!19} &  0.2045$^{\ddag}$ \cellcolor{green!32} &  0.2096$^{\ddag}$ \cellcolor{green!27} &  0.2687$^{\dag}$ \cellcolor{red!33} &  0.2293$^{\ddag}$ \cellcolor{green!7} & \textbf{0.2025}$^{\phantom{\ddag}}$ \cellcolor{green!35} \\\cline{2-12}
wine-q-white &  0.5107$^{\phantom{\ddag}}$ \cellcolor{red!35} &  0.3344$^{\phantom{\ddag}}$ \cellcolor{green!14} &  0.2853$^{\phantom{\ddag}}$ \cellcolor{green!28} &  0.3131$^{\phantom{\ddag}}$ \cellcolor{green!20} &  0.2638$^{\phantom{\ddag}}$ \cellcolor{green!34} &  0.2932$^{\phantom{\ddag}}$ \cellcolor{green!25} &  0.3885$^{\phantom{\ddag}}$ \cellcolor{red!0} &  0.3842$^{\phantom{\ddag}}$ \cellcolor{green!0} &  0.2667$^{\ddag}$ \cellcolor{green!33} & \textbf{0.2607}$^{\phantom{\ddag}}$ \cellcolor{green!35} &  0.2709$^{\phantom{\ddag}}$ \cellcolor{green!32} \\\cline{2-12}
yeast &  0.6177$^{\phantom{\ddag}}$ \cellcolor{red!35} &  0.4709$^{\phantom{\ddag}}$ \cellcolor{red!5} &  0.3914$^{\phantom{\ddag}}$ \cellcolor{green!9} &  0.2777$^{\phantom{\ddag}}$ \cellcolor{green!32} &  0.2842$^{\phantom{\ddag}}$ \cellcolor{green!31} & \textbf{0.2653}$^{\phantom{\ddag}}$ \cellcolor{green!35} &  0.4243$^{\phantom{\ddag}}$ \cellcolor{green!3} &  0.4118$^{\phantom{\ddag}}$ \cellcolor{green!5} &  0.4008$^{\phantom{\ddag}}$ \cellcolor{green!8} &  0.4434$^{\phantom{\ddag}}$ \cellcolor{red!0} &  0.3988$^{\dag}$ \cellcolor{green!8} \\\cline{2-12}
\hline 
 \textit{\textit{Average}} &  0.3405$^{\phantom{\ddag}}$ \cellcolor{red!14} &  0.2620$^{\phantom{\ddag}}$ \cellcolor{green!8} &  0.4067$^{\phantom{\ddag}}$ \cellcolor{red!35} &  0.2399$^{\phantom{\ddag}}$ \cellcolor{green!15} &  0.2618$^{\phantom{\ddag}}$ \cellcolor{green!8} & \textbf{0.1759}$^{\phantom{\ddag}}$ \cellcolor{green!35} &  0.2525$^{\phantom{\ddag}}$ \cellcolor{green!11} &  0.2383$^{\phantom{\ddag}}$ \cellcolor{green!16} &  0.3309$^{\phantom{\ddag}}$ \cellcolor{red!12} &  0.1921$^{\ddag}$ \cellcolor{green!30} &  0.1854$^{\dag}$ \cellcolor{green!32} \\\cline{2-12}
\textit{Rank} &  9.1 \cellcolor{red!35} &  7.9 \cellcolor{red!20} &  8.1 \cellcolor{red!23} &  4.8 \cellcolor{green!20} &  5.6 \cellcolor{green!9} &  3.7 \cellcolor{green!33} &  6.3 \cellcolor{green!0} &  5.3 \cellcolor{green!12} &  7.5 \cellcolor{red!15} & \textbf{3.6} \cellcolor{green!35} &  4.1 \cellcolor{green!27} \\\hline

\end{tabular}

==> tables/tab_ucimulti_mae.tex <==

            \begin{tabular}{|c|c|c|c|c||c|c||c|c||c|c|c|} \cline{2-12}
            \multicolumn{1}{c}{} & 
            \multicolumn{2}{|c}{Adjustment} & 
            \multicolumn{6}{|c|}{Distribution Matching} & 
            \multicolumn{3}{c|}{Maximum Likelihood} \\
             \cline{2-12} 
            \multicolumn{1}{c|}{} & ACC & PACC & HDy-OvA & DM-T & DM-HD & KDEy-HD & DM-CS & KDEy-CS & DIR & EMQ & KDEy-ML \rule{0pt}{10pt}   \\\hline
dry-bean & .0055$^{\phantom{\ddag}}$ \cellcolor{green!32} & .0050$^{\phantom{\ddag}}$ \cellcolor{green!33} & .0341$^{\phantom{\ddag}}$ \cellcolor{red!26} & .0048$^{\phantom{\ddag}}$ \cellcolor{green!33} & .0049$^{\phantom{\ddag}}$ \cellcolor{green!33} & .0066$^{\phantom{\ddag}}$ \cellcolor{green!30} & .0050$^{\phantom{\ddag}}$ \cellcolor{green!33} & .0049$^{\phantom{\ddag}}$ \cellcolor{green!33} & .0384$^{\phantom{\ddag}}$ \cellcolor{red!35} & .0056$^{\phantom{\ddag}}$ \cellcolor{green!32} & \textbf{.0043}$^{\phantom{\ddag}}$ \cellcolor{green!35} \\\hline
wine-quality & .1761$^{\phantom{\ddag}}$ \cellcolor{red!15} & .1697$^{\phantom{\ddag}}$ \cellcolor{red!12} & .1350$^{\phantom{\ddag}}$ \cellcolor{green!7} & .1449$^{\phantom{\ddag}}$ \cellcolor{green!1} & .1020$^{\phantom{\ddag}}$ \cellcolor{green!26} & \textbf{.0869}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .0894$^{\phantom{\ddag}}$ \cellcolor{green!33} & .1545$^{\phantom{\ddag}}$ \cellcolor{red!3} & .2093$^{\phantom{\ddag}}$ \cellcolor{red!35} & .1098$^{\phantom{\ddag}}$ \cellcolor{green!21} & .0984$^{\phantom{\ddag}}$ \cellcolor{green!28} \\\hline
academic-success & .0358$^{\phantom{\ddag}}$ \cellcolor{green!8} & .0286$^{\phantom{\ddag}}$ \cellcolor{green!22} & .0545$^{\phantom{\ddag}}$ \cellcolor{red!26} & .0230$^{\phantom{\ddag}}$ \cellcolor{green!32} & \textbf{.0218}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .0268$^{\phantom{\ddag}}$ \cellcolor{green!25} & .0282$^{\phantom{\ddag}}$ \cellcolor{green!22} & .0355$^{\phantom{\ddag}}$ \cellcolor{green!9} & .0589$^{\phantom{\ddag}}$ \cellcolor{red!35} & .0423$^{\phantom{\ddag}}$ \cellcolor{red!3} & .0240$^{\phantom{\ddag}}$ \cellcolor{green!30} \\\hline
digits & .0042$^{\phantom{\ddag}}$ \cellcolor{red!3} & .0037$^{\phantom{\ddag}}$ \cellcolor{green!7} & .0057$^{\phantom{\ddag}}$ \cellcolor{red!35} & .0030$^{\phantom{\ddag}}$ \cellcolor{green!23} & .0035$^{\phantom{\ddag}}$ \cellcolor{green!11} & .0051$^{\phantom{\ddag}}$ \cellcolor{red!22} & .0032$^{\phantom{\ddag}}$ \cellcolor{green!19} & .0030$^{\phantom{\ddag}}$ \cellcolor{green!23} & .0039$^{\phantom{\ddag}}$ \cellcolor{green!3} & .0025$^{\phantom{\ddag}}$ \cellcolor{green!33} & \textbf{.0024}$^{\phantom{\ddag}}$ \cellcolor{green!35} \\\hline
letter & .0062$^{\phantom{\ddag}}$ \cellcolor{green!18} & .0052$^{\phantom{\ddag}}$ \cellcolor{green!22} & .0181$^{\phantom{\ddag}}$ \cellcolor{red!35} & .0051$^{\phantom{\ddag}}$ \cellcolor{green!23} & .0054$^{\phantom{\ddag}}$ \cellcolor{green!21} & .0046$^{\phantom{\ddag}}$ \cellcolor{green!25} & .0071$^{\phantom{\ddag}}$ \cellcolor{green!13} & .0048$^{\phantom{\ddag}}$ \cellcolor{green!24} & .0093$^{\phantom{\ddag}}$ \cellcolor{green!4} & .0052$^{\phantom{\ddag}}$ \cellcolor{green!22} & \textbf{.0024}$^{\phantom{\ddag}}$ \cellcolor{green!35} \\\hline
\hline
Ave (MAE) & .0456$^{\phantom{\ddag}}$ \cellcolor{red!1} & .0424$^{\phantom{\ddag}}$ \cellcolor{green!4} & .0495$^{\phantom{\ddag}}$ \cellcolor{red!8} & .0362$^{\phantom{\ddag}}$ \cellcolor{green!16} & .0275$^{\phantom{\ddag}}$ \cellcolor{green!32} & \textbf{.0260}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .0266$^{\phantom{\ddag}}$ \cellcolor{green!33} & .0405$^{\phantom{\ddag}}$ \cellcolor{green!8} & .0640$^{\phantom{\ddag}}$ \cellcolor{red!35} & .0331$^{\phantom{\ddag}}$ \cellcolor{green!21} & .0263$^{\phantom{\ddag}}$ \cellcolor{green!34} \\\hline

\end{tabular}

==> tables/tab_ucimulti_mrae.tex <==

            \begin{tabular}{|c|c|c|c|c||c|c||c|c||c|c|c|} \cline{2-12}
            \multicolumn{1}{c}{} & 
            \multicolumn{2}{|c}{Adjustment} & 
            \multicolumn{6}{|c|}{Distribution Matching} & 
            \multicolumn{3}{c|}{Maximum Likelihood} \\
             \cline{2-12} 
            \multicolumn{1}{c|}{} & ACC & PACC & HDy-OvA & DM-T & DM-HD & KDEy-HD & DM-CS & KDEy-CS & DIR & EMQ & KDEy-ML \rule{0pt}{10pt}   \\\hline
dry-bean &  0.1070$^{\phantom{\ddag}}$ \cellcolor{green!33} &  0.0993$^{\phantom{\ddag}}$ \cellcolor{green!33} &  0.6775$^{\phantom{\ddag}}$ \cellcolor{red!0} &  0.0890$^{\phantom{\ddag}}$ \cellcolor{green!34} &  0.0868$^{\phantom{\ddag}}$ \cellcolor{green!34} &  0.1104$^{\phantom{\ddag}}$ \cellcolor{green!32} &  0.1049$^{\phantom{\ddag}}$ \cellcolor{green!33} &  0.0885$^{\phantom{\ddag}}$ \cellcolor{green!34} &  1.2572$^{\phantom{\ddag}}$ \cellcolor{red!35} &  0.0858$^{\phantom{\ddag}}$ \cellcolor{green!34} & \textbf{0.0732}$^{\phantom{\ddag}}$ \cellcolor{green!35} \\\hline
wine-quality &  3.9538$^{\phantom{\ddag}}$ \cellcolor{red!22} &  4.1116$^{\phantom{\ddag}}$ \cellcolor{red!27} &  3.2725$^{\phantom{\ddag}}$ \cellcolor{red!0} &  2.3474$^{\ddag}$ \cellcolor{green!28} &  2.1555$^{\ddag}$ \cellcolor{green!34} &  2.5102$^{\phantom{\ddag}}$ \cellcolor{green!23} &  2.9991$^{\phantom{\ddag}}$ \cellcolor{green!8} &  2.5214$^{\phantom{\ddag}}$ \cellcolor{green!23} &  4.3619$^{\phantom{\ddag}}$ \cellcolor{red!35} &  2.5655$^{\ddag}$ \cellcolor{green!21} & \textbf{2.1477}$^{\phantom{\ddag}}$ \cellcolor{green!35} \\\hline
academic-success &  0.4583$^{\phantom{\ddag}}$ \cellcolor{red!2} &  0.3175$^{\phantom{\ddag}}$ \cellcolor{green!15} &  0.5486$^{\phantom{\ddag}}$ \cellcolor{red!14} & \textbf{0.1611}$^{\phantom{\ddag}}$ \cellcolor{green!35} &  0.1704$^{\ddag}$ \cellcolor{green!33} &  0.2380$^{\phantom{\ddag}}$ \cellcolor{green!25} &  0.2237$^{\phantom{\ddag}}$ \cellcolor{green!27} &  0.2825$^{\phantom{\ddag}}$ \cellcolor{green!19} &  0.7133$^{\phantom{\ddag}}$ \cellcolor{red!35} &  0.2707$^{\phantom{\ddag}}$ \cellcolor{green!21} &  0.2067$^{\phantom{\ddag}}$ \cellcolor{green!29} \\\hline
digits &  0.1139$^{\phantom{\ddag}}$ \cellcolor{red!8} &  0.0851$^{\phantom{\ddag}}$ \cellcolor{green!11} &  0.1533$^{\phantom{\ddag}}$ \cellcolor{red!35} &  0.0574$^{\phantom{\ddag}}$ \cellcolor{green!29} &  0.0820$^{\phantom{\ddag}}$ \cellcolor{green!13} &  0.1154$^{\phantom{\ddag}}$ \cellcolor{red!9} &  0.1029$^{\phantom{\ddag}}$ \cellcolor{red!0} &  0.0556$^{\phantom{\ddag}}$ \cellcolor{green!31} &  0.1284$^{\phantom{\ddag}}$ \cellcolor{red!18} &  0.0512$^{\ddag}$ \cellcolor{green!34} & \textbf{0.0500}$^{\phantom{\ddag}}$ \cellcolor{green!35} \\\hline
letter &  0.3757$^{\phantom{\ddag}}$ \cellcolor{green!12} &  0.3158$^{\phantom{\ddag}}$ \cellcolor{green!18} &  0.8862$^{\phantom{\ddag}}$ \cellcolor{red!35} &  0.2567$^{\phantom{\ddag}}$ \cellcolor{green!23} &  0.2758$^{\phantom{\ddag}}$ \cellcolor{green!22} &  0.2571$^{\phantom{\ddag}}$ \cellcolor{green!23} &  0.5830$^{\phantom{\ddag}}$ \cellcolor{red!6} &  0.2427$^{\phantom{\ddag}}$ \cellcolor{green!25} &  0.7188$^{\phantom{\ddag}}$ \cellcolor{red!19} &  0.2612$^{\phantom{\ddag}}$ \cellcolor{green!23} & \textbf{0.1377}$^{\phantom{\ddag}}$ \cellcolor{green!35} \\\hline
\hline
Ave (MRAE) &  1.0017$^{\phantom{\ddag}}$ \cellcolor{red!1} &  0.9859$^{\phantom{\ddag}}$ \cellcolor{red!0} &  1.1076$^{\phantom{\ddag}}$ \cellcolor{red!9} &  0.5823$^{\phantom{\ddag}}$ \cellcolor{green!30} &  0.5541$^{\phantom{\ddag}}$ \cellcolor{green!32} &  0.6462$^{\phantom{\ddag}}$ \cellcolor{green!25} &  0.8027$^{\phantom{\ddag}}$ \cellcolor{green!13} &  0.6381$^{\phantom{\ddag}}$ \cellcolor{green!26} &  1.4359$^{\phantom{\ddag}}$ \cellcolor{red!35} &  0.6469$^{\phantom{\ddag}}$ \cellcolor{green!25} & \textbf{0.5231}$^{\phantom{\ddag}}$ \cellcolor{green!35} \\\hline

\end{tabular}

==> tables_sel/binary_mae.tex <==

            \begin{tabular}{|c|c|c|c|c|c|c|c|c|} \cline{2-9}           
            \multicolumn{1}{c}{} & 
            \multicolumn{1}{|c}{Adjustment} & 
            \multicolumn{5}{|c|}{Distribution Matching} & 
            \multicolumn{2}{c|}{Maximum Likelihood} \\
            \hline               
            \textbf{UCI-binary} & PACC & DM-T & DM-HD & KDEy-HD & DM-CS & KDEy-CS & EMQ & KDEy-ML \\\hline
\hline 
 \textit{Average} & .05679$^{\phantom{\ddag}}$ \cellcolor{red!35} & .05434$^{\phantom{\ddag}}$ \cellcolor{red!23} & .05647$^{\phantom{\ddag}}$ \cellcolor{red!33} & \textbf{.04249}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .04906$^{\phantom{\ddag}}$ \cellcolor{green!2} & .04956$^{\phantom{\ddag}}$ \cellcolor{green!0} & .05122$^{\phantom{\ddag}}$ \cellcolor{red!7} & .04529$^{\phantom{\ddag}}$ \cellcolor{green!21} \\\cline{2-9}

\textit{Rank} &  5.9 \cellcolor{red!35} &  4.4 \cellcolor{green!5} &  4.5 \cellcolor{green!5} & \textbf{3.4} \cellcolor{green!35} &  5.3 \cellcolor{red!19} &  5.0 \cellcolor{red!9} &  3.6 \cellcolor{green!29} &  3.9 \cellcolor{green!22} \\\hline
\hline
\textbf{LeQua} & PACC & DM-T & DM-HD & KDEy-HD & DM-CS & KDEy-CS & EMQ & KDEy-ML \\\hline
T1A & .02642$^{\phantom{\ddag}}$ \cellcolor{red!35} & .02364$^{\dag}$ \cellcolor{green!31} & .02371$^{\phantom{\ddag}}$ \cellcolor{green!29} & \textbf{.02350}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .02502$^{\phantom{\ddag}}$ \cellcolor{red!1} & .02473$^{\phantom{\ddag}}$ \cellcolor{green!5} & .02359$^{\ddag}$ \cellcolor{green!32} & .02417$^{\phantom{\ddag}}$ \cellcolor{green!18} \\\cline{2-9}

\textit{Rank} &  8 \cellcolor{red!35} &  3 \cellcolor{green!15} &  4 \cellcolor{green!4} & \textbf{1} \cellcolor{green!35} &  7 \cellcolor{red!24} &  6 \cellcolor{red!15} &  2 \cellcolor{green!25} &  5 \cellcolor{red!4} \\\hline

\end{tabular}

==> tables_sel/binary_mrae.tex <==

            \begin{tabular}{|c|c|c|c|c|c|c|c|c|} \cline{2-9}           
            \multicolumn{1}{c}{} & 
            \multicolumn{1}{|c}{Adjustment} & 
            \multicolumn{5}{|c|}{Distribution Matching} & 
            \multicolumn{2}{c|}{Maximum Likelihood} \\
            \hline               
            \textbf{UCI-binary} & PACC & DM-T & DM-HD & KDEy-HD & DM-CS & KDEy-CS & EMQ & KDEy-ML \\\hline
\hline 
 \textit{Average} &  0.26198$^{\phantom{\ddag}}$ \cellcolor{red!35} &  0.23992$^{\phantom{\ddag}}$ \cellcolor{red!17} &  0.26182$^{\phantom{\ddag}}$ \cellcolor{red!34} & \textbf{0.17587}$^{\phantom{\ddag}}$ \cellcolor{green!35} &  0.25255$^{\phantom{\ddag}}$ \cellcolor{red!27} &  0.23828$^{\phantom{\ddag}}$ \cellcolor{red!15} &  0.19214$^{\ddag}$ \cellcolor{green!21} &  0.18541$^{\dag}$ \cellcolor{green!27} \\\cline{2-9}

\textit{Rank} &  6.8 \cellcolor{red!35} &  4.2 \cellcolor{green!15} &  4.8 \cellcolor{green!3} & \textbf{3.2} \cellcolor{green!35} &  5.4 \cellcolor{red!8} &  4.6 \cellcolor{green!7} &  3.3 \cellcolor{green!34} &  3.6 \cellcolor{green!28} \\\hline
\hline
\textbf{LeQua} & PACC & DM-T & DM-HD & KDEy-HD & DM-CS & KDEy-CS & EMQ & KDEy-ML \\\hline
T1A &  0.16476$^{\phantom{\ddag}}$ \cellcolor{red!35} &  0.12019$^{\phantom{\ddag}}$ \cellcolor{green!20} &  0.11711$^{\phantom{\ddag}}$ \cellcolor{green!24} &  0.11766$^{\phantom{\ddag}}$ \cellcolor{green!23} &  0.14913$^{\phantom{\ddag}}$ \cellcolor{red!15} &  0.14167$^{\phantom{\ddag}}$ \cellcolor{red!6} & \textbf{0.10878}$^{\phantom{\ddag}}$ \cellcolor{green!35} &  0.11641$^{\phantom{\ddag}}$ \cellcolor{green!25} \\\cline{2-9}

\textit{Rank} &  8 \cellcolor{red!35} &  5 \cellcolor{red!4} &  3 \cellcolor{green!15} &  4 \cellcolor{green!4} &  7 \cellcolor{red!24} &  6 \cellcolor{red!15} & \textbf{1} \cellcolor{green!35} &  2 \cellcolor{green!25} \\\hline

\end{tabular}

==> tables_sel/ucibinary_mae.tex <==

            \begin{tabular}{|c|c|c|c|c|c|c|c|c|} \cline{2-9}           
            \multicolumn{1}{c}{} & 
            \multicolumn{1}{|c}{Adjustment} & 
            \multicolumn{5}{|c|}{Distribution Matching} & 
            \multicolumn{2}{c|}{Maximum Likelihood} \\
            \hline               
            \textbf{UCI-binary} & PACC & DM-T & DM-HD & KDEy-HD & DM-CS & KDEy-CS & EMQ & KDEy-ML \\\hline
balance.1 & \textbf{.01125}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .01358$^{\phantom{\ddag}}$ \cellcolor{green!31} & .01924$^{\phantom{\ddag}}$ \cellcolor{green!21} & .02146$^{\phantom{\ddag}}$ \cellcolor{green!17} & .03711$^{\phantom{\ddag}}$ \cellcolor{red!8} & .05275$^{\phantom{\ddag}}$ \cellcolor{red!35} & .02025$^{\phantom{\ddag}}$ \cellcolor{green!19} & .01825$^{\phantom{\ddag}}$ \cellcolor{green!23} \\\cline{2-9}
balance.3 & \textbf{.01855}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .02847$^{\phantom{\ddag}}$ \cellcolor{red!35} & .01889$^{\ddag}$ \cellcolor{green!32} & .02109$^{\phantom{\ddag}}$ \cellcolor{green!17} & .02396$^{\phantom{\ddag}}$ \cellcolor{red!3} & .02422$^{\phantom{\ddag}}$ \cellcolor{red!5} & .02420$^{\phantom{\ddag}}$ \cellcolor{red!4} & .02372$^{\phantom{\ddag}}$ \cellcolor{red!1} \\\cline{2-9}
breast-cancer & .02360$^{\phantom{\ddag}}$ \cellcolor{red!31} & .01731$^{\phantom{\ddag}}$ \cellcolor{red!4} & .02434$^{\phantom{\ddag}}$ \cellcolor{red!35} & .02028$^{\phantom{\ddag}}$ \cellcolor{red!17} & .00976$^{\phantom{\ddag}}$ \cellcolor{green!27} & \textbf{.00800}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .00895$^{\phantom{\ddag}}$ \cellcolor{green!30} & .01311$^{\phantom{\ddag}}$ \cellcolor{green!13} \\\cline{2-9}
cmc.1 & \textbf{.08625}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .09403$^{\phantom{\ddag}}$ \cellcolor{green!19} & .09622$^{\phantom{\ddag}}$ \cellcolor{green!15} & .09223$^{\phantom{\ddag}}$ \cellcolor{green!23} & .12185$^{\phantom{\ddag}}$ \cellcolor{red!35} & .10372$^{\phantom{\ddag}}$ \cellcolor{green!0} & .09124$^{\phantom{\ddag}}$ \cellcolor{green!25} & .09736$^{\phantom{\ddag}}$ \cellcolor{green!13} \\\cline{2-9}
cmc.2 & .10111$^{\phantom{\ddag}}$ \cellcolor{green!15} & .17772$^{\phantom{\ddag}}$ \cellcolor{red!31} & .18373$^{\phantom{\ddag}}$ \cellcolor{red!35} & .08614$^{\phantom{\ddag}}$ \cellcolor{green!25} & .08641$^{\phantom{\ddag}}$ \cellcolor{green!24} & .07881$^{\phantom{\ddag}}$ \cellcolor{green!29} & \textbf{.07000}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .08788$^{\phantom{\ddag}}$ \cellcolor{green!23} \\\cline{2-9}
cmc.3 & .13990$^{\phantom{\ddag}}$ \cellcolor{red!13} & .13005$^{\phantom{\ddag}}$ \cellcolor{green!12} & \textbf{.12160}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .12377$^{\ddag}$ \cellcolor{green!29} & .14353$^{\phantom{\ddag}}$ \cellcolor{red!22} & .14828$^{\phantom{\ddag}}$ \cellcolor{red!35} & .12717$^{\ddag}$ \cellcolor{green!20} & .12330$^{\ddag}$ \cellcolor{green!30} \\\cline{2-9}
ctg.1 & .01921$^{\phantom{\ddag}}$ \cellcolor{green!0} & .01847$^{\phantom{\ddag}}$ \cellcolor{green!6} & .01826$^{\phantom{\ddag}}$ \cellcolor{green!8} & .01751$^{\phantom{\ddag}}$ \cellcolor{green!15} & .01786$^{\phantom{\ddag}}$ \cellcolor{green!12} & .02317$^{\phantom{\ddag}}$ \cellcolor{red!35} & \textbf{.01526}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .01607$^{\dag}$ \cellcolor{green!27} \\\cline{2-9}
ctg.2 & .03317$^{\phantom{\ddag}}$ \cellcolor{red!35} & .01845$^{\ddag}$ \cellcolor{green!32} & .01862$^{\ddag}$ \cellcolor{green!31} & .01798$^{\ddag}$ \cellcolor{green!34} & .02012$^{\phantom{\ddag}}$ \cellcolor{green!24} & .01920$^{\phantom{\ddag}}$ \cellcolor{green!28} & \textbf{.01780}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .01935$^{\phantom{\ddag}}$ \cellcolor{green!27} \\\cline{2-9}
ctg.3 & .05073$^{\phantom{\ddag}}$ \cellcolor{red!19} & .03806$^{\phantom{\ddag}}$ \cellcolor{green!1} & .02972$^{\phantom{\ddag}}$ \cellcolor{green!15} & .02911$^{\phantom{\ddag}}$ \cellcolor{green!16} & \textbf{.01820}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .01864$^{\ddag}$ \cellcolor{green!34} & .05973$^{\phantom{\ddag}}$ \cellcolor{red!35} & .02543$^{\phantom{\ddag}}$ \cellcolor{green!22} \\\cline{2-9}
german & .05913$^{\phantom{\ddag}}$ \cellcolor{green!24} & .07001$^{\phantom{\ddag}}$ \cellcolor{green!9} & .07002$^{\phantom{\ddag}}$ \cellcolor{green!9} & .06507$^{\phantom{\ddag}}$ \cellcolor{green!15} & .05341$^{\phantom{\ddag}}$ \cellcolor{green!32} & \textbf{.05129}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .10180$^{\phantom{\ddag}}$ \cellcolor{red!35} & .08384$^{\phantom{\ddag}}$ \cellcolor{red!10} \\\cline{2-9}
haberman & .15689$^{\phantom{\ddag}}$ \cellcolor{green!19} & .30098$^{\phantom{\ddag}}$ \cellcolor{red!19} & .36011$^{\phantom{\ddag}}$ \cellcolor{red!35} & \textbf{.09742}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .12137$^{\phantom{\ddag}}$ \cellcolor{green!28} & .18291$^{\phantom{\ddag}}$ \cellcolor{green!12} & .13554$^{\phantom{\ddag}}$ \cellcolor{green!24} & .12167$^{\phantom{\ddag}}$ \cellcolor{green!28} \\\cline{2-9}
ionosphere & .05077$^{\phantom{\ddag}}$ \cellcolor{green!15} & .03729$^{\phantom{\ddag}}$ \cellcolor{green!31} & .04210$^{\phantom{\ddag}}$ \cellcolor{green!25} & \textbf{.03441}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .09228$^{\phantom{\ddag}}$ \cellcolor{red!35} & .07849$^{\phantom{\ddag}}$ \cellcolor{red!18} & .03466$^{\ddag}$ \cellcolor{green!34} & .06550$^{\phantom{\ddag}}$ \cellcolor{red!2} \\\cline{2-9}
iris.2 & .08910$^{\phantom{\ddag}}$ \cellcolor{red!26} & .02508$^{\phantom{\ddag}}$ \cellcolor{green!33} & .03726$^{\phantom{\ddag}}$ \cellcolor{green!21} & .03905$^{\phantom{\ddag}}$ \cellcolor{green!20} & .03841$^{\phantom{\ddag}}$ \cellcolor{green!20} & \textbf{.02314}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .09805$^{\phantom{\ddag}}$ \cellcolor{red!35} & .03034$^{\phantom{\ddag}}$ \cellcolor{green!28} \\\cline{2-9}
iris.3 & \textbf{.06269}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .06778$^{\phantom{\ddag}}$ \cellcolor{red!24} & .06777$^{\phantom{\ddag}}$ \cellcolor{red!24} & .06686$^{\phantom{\ddag}}$ \cellcolor{red!13} & .06781$^{\phantom{\ddag}}$ \cellcolor{red!24} & .06483$^{\phantom{\ddag}}$ \cellcolor{green!9} & .06276$^{\ddag}$ \cellcolor{green!34} & .06868$^{\phantom{\ddag}}$ \cellcolor{red!35} \\\cline{2-9}
mammographic & .04319$^{\phantom{\ddag}}$ \cellcolor{red!4} & .04238$^{\phantom{\ddag}}$ \cellcolor{green!2} & .04264$^{\phantom{\ddag}}$ \cellcolor{green!0} & .04378$^{\phantom{\ddag}}$ \cellcolor{red!10} & \textbf{.03881}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .04650$^{\phantom{\ddag}}$ \cellcolor{red!35} & .04248$^{\phantom{\ddag}}$ \cellcolor{green!1} & .04001$^{\dag}$ \cellcolor{green!24} \\\cline{2-9}
pageblocks.5 & .02209$^{\phantom{\ddag}}$ \cellcolor{red!27} & .02234$^{\phantom{\ddag}}$ \cellcolor{red!30} & .02061$^{\phantom{\ddag}}$ \cellcolor{red!10} & .01950$^{\phantom{\ddag}}$ \cellcolor{green!2} & .02275$^{\phantom{\ddag}}$ \cellcolor{red!35} & .02052$^{\phantom{\ddag}}$ \cellcolor{red!9} & \textbf{.01667}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .01886$^{\phantom{\ddag}}$ \cellcolor{green!9} \\\cline{2-9}
semeion & .03079$^{\phantom{\ddag}}$ \cellcolor{red!35} & .01703$^{\phantom{\ddag}}$ \cellcolor{green!16} & .01987$^{\phantom{\ddag}}$ \cellcolor{green!6} & .01498$^{\phantom{\ddag}}$ \cellcolor{green!24} & .01760$^{\phantom{\ddag}}$ \cellcolor{green!14} & .01792$^{\phantom{\ddag}}$ \cellcolor{green!13} & \textbf{.01215}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .01796$^{\phantom{\ddag}}$ \cellcolor{green!13} \\\cline{2-9}
sonar & .15535$^{\phantom{\ddag}}$ \cellcolor{red!35} & .06595$^{\phantom{\ddag}}$ \cellcolor{green!24} & .06867$^{\phantom{\ddag}}$ \cellcolor{green!22} & \textbf{.04994}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .06179$^{\phantom{\ddag}}$ \cellcolor{green!27} & .05253$^{\dag}$ \cellcolor{green!33} & .06729$^{\phantom{\ddag}}$ \cellcolor{green!23} & .05860$^{\phantom{\ddag}}$ \cellcolor{green!29} \\\cline{2-9}
spambase & .02058$^{\phantom{\ddag}}$ \cellcolor{red!35} & .01894$^{\dag}$ \cellcolor{green!16} & .01908$^{\dag}$ \cellcolor{green!12} & .01865$^{\ddag}$ \cellcolor{green!25} & .02030$^{\phantom{\ddag}}$ \cellcolor{red!26} & .01945$^{\phantom{\ddag}}$ \cellcolor{green!0} & .01945$^{\phantom{\ddag}}$ \cellcolor{green!0} & \textbf{.01836}$^{\phantom{\ddag}}$ \cellcolor{green!35} \\\cline{2-9}
spectf & .05076$^{\phantom{\ddag}}$ \cellcolor{green!22} & .04095$^{\phantom{\ddag}}$ \cellcolor{green!31} & .04095$^{\phantom{\ddag}}$ \cellcolor{green!31} & \textbf{.03623}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .04413$^{\phantom{\ddag}}$ \cellcolor{green!28} & .04334$^{\phantom{\ddag}}$ \cellcolor{green!29} & .12048$^{\phantom{\ddag}}$ \cellcolor{red!35} & .04391$^{\phantom{\ddag}}$ \cellcolor{green!28} \\\cline{2-9}
tictactoe & .00905$^{\phantom{\ddag}}$ \cellcolor{green!2} & .00833$^{\phantom{\ddag}}$ \cellcolor{green!16} & .00778$^{\phantom{\ddag}}$ \cellcolor{green!27} & .00827$^{\phantom{\ddag}}$ \cellcolor{green!17} & \textbf{.00740}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .00760$^{\ddag}$ \cellcolor{green!30} & .00746$^{\ddag}$ \cellcolor{green!33} & .01093$^{\phantom{\ddag}}$ \cellcolor{red!35} \\\cline{2-9}
transfusion & .08166$^{\phantom{\ddag}}$ \cellcolor{red!35} & .07376$^{\phantom{\ddag}}$ \cellcolor{green!0} & .07381$^{\phantom{\ddag}}$ \cellcolor{green!0} & \textbf{.06597}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .07609$^{\phantom{\ddag}}$ \cellcolor{red!10} & .07328$^{\phantom{\ddag}}$ \cellcolor{green!2} & .06775$^{\phantom{\ddag}}$ \cellcolor{green!27} & .07195$^{\phantom{\ddag}}$ \cellcolor{green!8} \\\cline{2-9}
wdbc & .01690$^{\phantom{\ddag}}$ \cellcolor{red!16} & \textbf{.01076}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .01206$^{\phantom{\ddag}}$ \cellcolor{green!23} & .01364$^{\phantom{\ddag}}$ \cellcolor{green!10} & .01617$^{\phantom{\ddag}}$ \cellcolor{red!10} & .01884$^{\phantom{\ddag}}$ \cellcolor{red!33} & .01298$^{\phantom{\ddag}}$ \cellcolor{green!16} & .01904$^{\phantom{\ddag}}$ \cellcolor{red!35} \\\cline{2-9}
wine.1 & .03781$^{\phantom{\ddag}}$ \cellcolor{red!35} & .02190$^{\phantom{\ddag}}$ \cellcolor{green!3} & \textbf{.00851}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .01334$^{\phantom{\ddag}}$ \cellcolor{green!23} & .02221$^{\phantom{\ddag}}$ \cellcolor{green!2} & .02124$^{\phantom{\ddag}}$ \cellcolor{green!4} & .01299$^{\phantom{\ddag}}$ \cellcolor{green!24} & .00962$^{\phantom{\ddag}}$ \cellcolor{green!32} \\\cline{2-9}
wine.2 & .02417$^{\phantom{\ddag}}$ \cellcolor{red!35} & .01076$^{\phantom{\ddag}}$ \cellcolor{green!24} & .01092$^{\phantom{\ddag}}$ \cellcolor{green!23} & .01142$^{\phantom{\ddag}}$ \cellcolor{green!21} & .01203$^{\phantom{\ddag}}$ \cellcolor{green!18} & .01148$^{\phantom{\ddag}}$ \cellcolor{green!20} & .00936$^{\phantom{\ddag}}$ \cellcolor{green!30} & \textbf{.00831}$^{\phantom{\ddag}}$ \cellcolor{green!35} \\\cline{2-9}
wine.3 & .02997$^{\phantom{\ddag}}$ \cellcolor{red!35} & .01439$^{\phantom{\ddag}}$ \cellcolor{green!20} & .01760$^{\phantom{\ddag}}$ \cellcolor{green!9} & .01276$^{\phantom{\ddag}}$ \cellcolor{green!26} & .02422$^{\phantom{\ddag}}$ \cellcolor{red!14} & .02337$^{\phantom{\ddag}}$ \cellcolor{red!11} & .01733$^{\phantom{\ddag}}$ \cellcolor{green!10} & \textbf{.01040}$^{\phantom{\ddag}}$ \cellcolor{green!35} \\\cline{2-9}
wine-q-red & .04968$^{\ddag}$ \cellcolor{green!23} & .04943$^{\phantom{\ddag}}$ \cellcolor{green!25} & .04957$^{\phantom{\ddag}}$ \cellcolor{green!24} & .05926$^{\phantom{\ddag}}$ \cellcolor{red!35} & .05595$^{\phantom{\ddag}}$ \cellcolor{red!14} & .05427$^{\phantom{\ddag}}$ \cellcolor{red!4} & .04785$^{\ddag}$ \cellcolor{green!34} & \textbf{.04781}$^{\phantom{\ddag}}$ \cellcolor{green!35} \\\cline{2-9}
wine-q-white & .06748$^{\phantom{\ddag}}$ \cellcolor{green!11} & .07032$^{\phantom{\ddag}}$ \cellcolor{red!9} & .06685$^{\phantom{\ddag}}$ \cellcolor{green!15} & .06945$^{\phantom{\ddag}}$ \cellcolor{red!2} & .07032$^{\phantom{\ddag}}$ \cellcolor{red!9} & .07399$^{\phantom{\ddag}}$ \cellcolor{red!35} & \textbf{.06409}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .06559$^{\phantom{\ddag}}$ \cellcolor{green!24} \\\cline{2-9}
yeast & .10517$^{\phantom{\ddag}}$ \cellcolor{red!35} & .07149$^{\phantom{\ddag}}$ \cellcolor{green!20} & .07077$^{\phantom{\ddag}}$ \cellcolor{green!21} & \textbf{.06255}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .08089$^{\phantom{\ddag}}$ \cellcolor{green!4} & .07534$^{\phantom{\ddag}}$ \cellcolor{green!13} & .09952$^{\phantom{\ddag}}$ \cellcolor{red!25} & .07758$^{\phantom{\ddag}}$ \cellcolor{green!10} \\\cline{2-9}
\hline 
 \textit{Average} & .05679$^{\phantom{\ddag}}$ \cellcolor{red!35} & .05434$^{\phantom{\ddag}}$ \cellcolor{red!23} & .05647$^{\phantom{\ddag}}$ \cellcolor{red!33} & \textbf{.04249}$^{\phantom{\ddag}}$ \cellcolor{green!35} & .04906$^{\phantom{\ddag}}$ \cellcolor{green!2} & .04956$^{\phantom{\ddag}}$ \cellcolor{green!0} & .05122$^{\phantom{\ddag}}$ \cellcolor{red!7} & .04529$^{\phantom{\ddag}}$ \cellcolor{green!21} \\\cline{2-9}
\textit{Rank} &  5.9 \cellcolor{red!35} &  4.4 \cellcolor{green!5} &  4.5 \cellcolor{green!5} & \textbf{3.4} \cellcolor{green!35} &  5.3 \cellcolor{red!19} &  5.0 \cellcolor{red!9} &  3.6 \cellcolor{green!29} &  3.9 \cellcolor{green!22} \\\hline

\end{tabular}

==> tables_sel/ucibinary_mrae.tex <==

            \begin{tabular}{|c|c|c|c|c|c|c|c|c|} \cline{2-9}           
            \multicolumn{1}{c}{} & 
            \multicolumn{1}{|c}{Adjustment} & 
            \multicolumn{5}{|c|}{Distribution Matching} & 
            \multicolumn{2}{c|}{Maximum Likelihood} \\
            \hline               
            \textbf{UCI-binary} & PACC & DM-T & DM-HD & KDEy-HD & DM-CS & KDEy-CS & EMQ & KDEy-ML \\\hline
balance.1 &  0.05394$^{\phantom{\ddag}}$ \cellcolor{green!32} & \textbf{0.05070}$^{\phantom{\ddag}}$ \cellcolor{green!35} &  0.07789$^{\phantom{\ddag}}$ \cellcolor{green!17} &  0.07458$^{\phantom{\ddag}}$ \cellcolor{green!19} &  0.15757$^{\phantom{\ddag}}$ \cellcolor{red!35} &  0.14958$^{\phantom{\ddag}}$ \cellcolor{red!29} &  0.06760$^{\phantom{\ddag}}$ \cellcolor{green!23} &  0.09535$^{\phantom{\ddag}}$ \cellcolor{green!5} \\\cline{2-9}
balance.3 &  0.11497$^{\phantom{\ddag}}$ \cellcolor{green!2} & \textbf{0.09061}$^{\phantom{\ddag}}$ \cellcolor{green!35} &  0.11132$^{\phantom{\ddag}}$ \cellcolor{green!7} &  0.10595$^{\ddag}$ \cellcolor{green!14} &  0.14388$^{\phantom{\ddag}}$ \cellcolor{red!35} &  0.12839$^{\phantom{\ddag}}$ \cellcolor{red!14} &  0.10724$^{\phantom{\ddag}}$ \cellcolor{green!13} &  0.11134$^{\dag}$ \cellcolor{green!7} \\\cline{2-9}
breast-cancer &  0.11482$^{\phantom{\ddag}}$ \cellcolor{red!35} &  0.07536$^{\phantom{\ddag}}$ \cellcolor{green!0} &  0.09187$^{\phantom{\ddag}}$ \cellcolor{red!14} &  0.07237$^{\phantom{\ddag}}$ \cellcolor{green!2} &  0.04959$^{\phantom{\ddag}}$ \cellcolor{green!23} &  0.04249$^{\phantom{\ddag}}$ \cellcolor{green!29} & \textbf{0.03660}$^{\phantom{\ddag}}$ \cellcolor{green!35} &  0.03825$^{\phantom{\ddag}}$ \cellcolor{green!33} \\\cline{2-9}
cmc.1 &  0.40790$^{\phantom{\ddag}}$ \cellcolor{red!3} &  0.33894$^{\phantom{\ddag}}$ \cellcolor{green!29} &  0.34912$^{\phantom{\ddag}}$ \cellcolor{green!24} & \textbf{0.32662}$^{\phantom{\ddag}}$ \cellcolor{green!35} &  0.47610$^{\phantom{\ddag}}$ \cellcolor{red!35} &  0.37953$^{\phantom{\ddag}}$ \cellcolor{green!10} &  0.34765$^{\phantom{\ddag}}$ \cellcolor{green!25} &  0.33036$^{\phantom{\ddag}}$ \cellcolor{green!33} \\\cline{2-9}
cmc.2 &  0.44461$^{\phantom{\ddag}}$ \cellcolor{green!14} &  0.79129$^{\phantom{\ddag}}$ \cellcolor{red!35} &  0.78553$^{\phantom{\ddag}}$ \cellcolor{red!34} &  0.35677$^{\dag}$ \cellcolor{green!27} &  0.69000$^{\phantom{\ddag}}$ \cellcolor{red!20} &  0.58605$^{\phantom{\ddag}}$ \cellcolor{red!5} & \textbf{0.30444}$^{\phantom{\ddag}}$ \cellcolor{green!35} &  0.31391$^{\phantom{\ddag}}$ \cellcolor{green!33} \\\cline{2-9}
cmc.3 &  0.67741$^{\phantom{\ddag}}$ \cellcolor{red!35} &  0.43845$^{\ddag}$ \cellcolor{green!23} &  0.42377$^{\ddag}$ \cellcolor{green!27} &  0.41053$^{\phantom{\ddag}}$ \cellcolor{green!30} &  0.52581$^{\phantom{\ddag}}$ \cellcolor{green!2} &  0.48838$^{\phantom{\ddag}}$ \cellcolor{green!11} &  0.41600$^{\ddag}$ \cellcolor{green!29} & \textbf{0.39327}$^{\phantom{\ddag}}$ \cellcolor{green!35} \\\cline{2-9}
ctg.1 &  0.09070$^{\phantom{\ddag}}$ \cellcolor{red!35} &  0.06919$^{\phantom{\ddag}}$ \cellcolor{green!14} &  0.06860$^{\phantom{\ddag}}$ \cellcolor{green!15} &  0.06594$^{\phantom{\ddag}}$ \cellcolor{green!21} &  0.08054$^{\phantom{\ddag}}$ \cellcolor{red!11} &  0.07822$^{\phantom{\ddag}}$ \cellcolor{red!6} & \textbf{0.06000}$^{\phantom{\ddag}}$ \cellcolor{green!35} &  0.06267$^{\ddag}$ \cellcolor{green!28} \\\cline{2-9}
ctg.2 &  0.17255$^{\phantom{\ddag}}$ \cellcolor{red!35} &  0.09506$^{\ddag}$ \cellcolor{green!28} &  0.09565$^{\ddag}$ \cellcolor{green!27} &  0.08988$^{\ddag}$ \cellcolor{green!32} &  0.09545$^{\phantom{\ddag}}$ \cellcolor{green!27} &  0.09703$^{\dag}$ \cellcolor{green!26} & \textbf{0.08684}$^{\phantom{\ddag}}$ \cellcolor{green!35} &  0.09802$^{\ddag}$ \cellcolor{green!25} \\\cline{2-9}
ctg.3 &  0.23311$^{\phantom{\ddag}}$ \cellcolor{red!35} &  0.12351$^{\phantom{\ddag}}$ \cellcolor{green!11} &  0.18102$^{\phantom{\ddag}}$ \cellcolor{red!13} &  0.12668$^{\phantom{\ddag}}$ \cellcolor{green!9} &  0.07125$^{\phantom{\ddag}}$ \cellcolor{green!33} & \textbf{0.06693}$^{\phantom{\ddag}}$ \cellcolor{green!35} &  0.07292$^{\ddag}$ \cellcolor{green!32} &  0.09961$^{\phantom{\ddag}}$ \cellcolor{green!21} \\\cline{2-9}
german &  0.30472$^{\phantom{\ddag}}$ \cellcolor{green!9} &  0.22694$^{\phantom{\ddag}}$ \cellcolor{green!30} &  0.46656$^{\phantom{\ddag}}$ \cellcolor{red!35} &  0.23917$^{\phantom{\ddag}}$ \cellcolor{green!26} &  0.21290$^{\phantom{\ddag}}$ \cellcolor{green!34} & \textbf{0.20972}$^{\phantom{\ddag}}$ \cellcolor{green!35} &  0.33776$^{\phantom{\ddag}}$ \cellcolor{green!0} &  0.30216$^{\phantom{\ddag}}$ \cellcolor{green!9} \\\cline{2-9}
haberman &  0.50400$^{\phantom{\ddag}}$ \cellcolor{green!29} &  1.59175$^{\phantom{\ddag}}$ \cellcolor{red!21} &  1.87374$^{\phantom{\ddag}}$ \cellcolor{red!35} & \textbf{0.38303}$^{\phantom{\ddag}}$ \cellcolor{green!35} &  1.17885$^{\phantom{\ddag}}$ \cellcolor{red!2} &  1.18703$^{\phantom{\ddag}}$ \cellcolor{red!2} &  0.40947$^{\phantom{\ddag}}$ \cellcolor{green!33} &  0.41646$^{\phantom{\ddag}}$ \cellcolor{green!33} \\\cline{2-9}
ionosphere &  0.24006$^{\phantom{\ddag}}$ \cellcolor{green!15} & \textbf{0.13774}$^{\phantom{\ddag}}$ \cellcolor{green!35} &  0.14993$^{\phantom{\ddag}}$ \cellcolor{green!32} &  0.14287$^{\phantom{\ddag}}$ \cellcolor{green!34} &  0.49831$^{\phantom{\ddag}}$ \cellcolor{red!35} &  0.41450$^{\phantom{\ddag}}$ \cellcolor{red!18} &  0.18468$^{\ddag}$ \cellcolor{green!25} &  0.36913$^{\phantom{\ddag}}$ \cellcolor{red!9} \\\cline{2-9}
iris.2 &  0.32526$^{\phantom{\ddag}}$ \cellcolor{red!6} &  0.17372$^{\phantom{\ddag}}$ \cellcolor{green!22} &  0.13826$^{\phantom{\ddag}}$ \cellcolor{green!29} &  0.12597$^{\phantom{\ddag}}$ \cellcolor{green!32} &  0.18014$^{\phantom{\ddag}}$ \cellcolor{green!21} &  0.12498$^{\phantom{\ddag}}$ \cellcolor{green!32} &  0.47648$^{\phantom{\ddag}}$ \cellcolor{red!35} & \textbf{0.11035}$^{\phantom{\ddag}}$ \cellcolor{green!35} \\\cline{2-9}
iris.3 &  0.33284$^{\ddag}$ \cellcolor{green!32} &  0.37974$^{\phantom{\ddag}}$ \cellcolor{red!19} &  0.37933$^{\phantom{\ddag}}$ \cellcolor{red!18} &  0.36952$^{\phantom{\ddag}}$ \cellcolor{red!7} &  0.37954$^{\phantom{\ddag}}$ \cellcolor{red!18} &  0.36225$^{\phantom{\ddag}}$ \cellcolor{green!0} & \textbf{0.33049}$^{\phantom{\ddag}}$ \cellcolor{green!35} &  0.39412$^{\phantom{\ddag}}$ \cellcolor{red!35} \\\cline{2-9}
mammographic &  0.29023$^{\phantom{\ddag}}$ \cellcolor{red!35} &  0.23843$^{\phantom{\ddag}}$ \cellcolor{red!3} &  0.23732$^{\phantom{\ddag}}$ \cellcolor{red!3} &  0.25063$^{\phantom{\ddag}}$ \cellcolor{red!11} &  0.25182$^{\phantom{\ddag}}$ \cellcolor{red!11} &  0.26240$^{\phantom{\ddag}}$ \cellcolor{red!18} & \textbf{0.17420}$^{\phantom{\ddag}}$ \cellcolor{green!35} &  0.17949$^{\phantom{\ddag}}$ \cellcolor{green!31} \\\cline{2-9}
pageblocks.5 &  0.11171$^{\phantom{\ddag}}$ \cellcolor{red!35} &  0.09612$^{\phantom{\ddag}}$ \cellcolor{green!9} &  0.08858$^{\ddag}$ \cellcolor{green!30} & \textbf{0.08695}$^{\phantom{\ddag}}$ \cellcolor{green!35} &  0.08941$^{\dag}$ \cellcolor{green!28} &  0.08708$^{\ddag}$ \cellcolor{green!34} &  0.09617$^{\phantom{\ddag}}$ \cellcolor{green!8} &  0.09144$^{\phantom{\ddag}}$ \cellcolor{green!22} \\\cline{2-9}
semeion &  0.17288$^{\phantom{\ddag}}$ \cellcolor{red!28} &  0.16026$^{\phantom{\ddag}}$ \cellcolor{red!21} &  0.18683$^{\phantom{\ddag}}$ \cellcolor{red!35} &  0.06313$^{\phantom{\ddag}}$ \cellcolor{green!26} &  0.07645$^{\phantom{\ddag}}$ \cellcolor{green!19} &  0.06755$^{\phantom{\ddag}}$ \cellcolor{green!24} & \textbf{0.04577}$^{\phantom{\ddag}}$ \cellcolor{green!35} &  0.06940$^{\phantom{\ddag}}$ \cellcolor{green!23} \\\cline{2-9}
sonar &  0.59209$^{\phantom{\ddag}}$ \cellcolor{red!35} &  0.22124$^{\phantom{\ddag}}$ \cellcolor{green!26} &  0.22782$^{\phantom{\ddag}}$ \cellcolor{green!25} & \textbf{0.17289}$^{\phantom{\ddag}}$ \cellcolor{green!35} &  0.22830$^{\phantom{\ddag}}$ \cellcolor{green!25} &  0.21346$^{\phantom{\ddag}}$ \cellcolor{green!28} &  0.34445$^{\phantom{\ddag}}$ \cellcolor{green!6} &  0.19494$^{\phantom{\ddag}}$ \cellcolor{green!31} \\\cline{2-9}
spambase &  0.09588$^{\phantom{\ddag}}$ \cellcolor{red!35} & \textbf{0.08206}$^{\phantom{\ddag}}$ \cellcolor{green!35} &  0.08218$^{\ddag}$ \cellcolor{green!34} &  0.08247$^{\ddag}$ \cellcolor{green!32} &  0.08953$^{\phantom{\ddag}}$ \cellcolor{red!2} &  0.08565$^{\phantom{\ddag}}$ \cellcolor{green!16} &  0.09334$^{\dag}$ \cellcolor{red!22} &  0.08302$^{\ddag}$ \cellcolor{green!30} \\\cline{2-9}
spectf &  0.33522$^{\phantom{\ddag}}$ \cellcolor{red!35} &  0.18082$^{\phantom{\ddag}}$ \cellcolor{green!22} &  0.19621$^{\phantom{\ddag}}$ \cellcolor{green!16} & \textbf{0.14596}$^{\phantom{\ddag}}$ \cellcolor{green!35} &  0.18122$^{\phantom{\ddag}}$ \cellcolor{green!21} &  0.17453$^{\phantom{\ddag}}$ \cellcolor{green!24} &  0.15283$^{\phantom{\ddag}}$ \cellcolor{green!32} &  0.16363$^{\phantom{\ddag}}$ \cellcolor{green!28} \\\cline{2-9}
tictactoe &  0.03911$^{\phantom{\ddag}}$ \cellcolor{red!17} &  0.03596$^{\phantom{\ddag}}$ \cellcolor{green!2} &  0.04190$^{\phantom{\ddag}}$ \cellcolor{red!35} &  0.03262$^{\phantom{\ddag}}$ \cellcolor{green!24} &  0.03262$^{\ddag}$ \cellcolor{green!24} &  0.03138$^{\ddag}$ \cellcolor{green!32} & \textbf{0.03092}$^{\phantom{\ddag}}$ \cellcolor{green!35} &  0.03597$^{\dag}$ \cellcolor{green!2} \\\cline{2-9}
transfusion &  0.40587$^{\phantom{\ddag}}$ \cellcolor{red!35} &  0.28794$^{\ddag}$ \cellcolor{green!21} &  0.28768$^{\ddag}$ \cellcolor{green!22} &  0.29478$^{\phantom{\ddag}}$ \cellcolor{green!18} &  0.32646$^{\phantom{\ddag}}$ \cellcolor{green!3} &  0.38365$^{\ddag}$ \cellcolor{red!24} & \textbf{0.26102}$^{\phantom{\ddag}}$ \cellcolor{green!35} &  0.33877$^{\phantom{\ddag}}$ \cellcolor{red!2} \\\cline{2-9}
wdbc &  0.11053$^{\phantom{\ddag}}$ \cellcolor{red!35} &  0.05068$^{\dag}$ \cellcolor{green!34} & \textbf{0.05029}$^{\phantom{\ddag}}$ \cellcolor{green!35} &  0.08002$^{\phantom{\ddag}}$ \cellcolor{green!0} &  0.06259$^{\phantom{\ddag}}$ \cellcolor{green!20} &  0.06356$^{\phantom{\ddag}}$ \cellcolor{green!19} &  0.06334$^{\phantom{\ddag}}$ \cellcolor{green!19} &  0.08086$^{\phantom{\ddag}}$ \cellcolor{red!0} \\\cline{2-9}
wine.1 &  0.16758$^{\phantom{\ddag}}$ \cellcolor{red!35} &  0.10045$^{\phantom{\ddag}}$ \cellcolor{green!4} &  0.11713$^{\phantom{\ddag}}$ \cellcolor{red!5} &  0.06193$^{\phantom{\ddag}}$ \cellcolor{green!26} &  0.09921$^{\phantom{\ddag}}$ \cellcolor{green!5} &  0.10123$^{\phantom{\ddag}}$ \cellcolor{green!3} &  0.05039$^{\phantom{\ddag}}$ \cellcolor{green!33} & \textbf{0.04826}$^{\phantom{\ddag}}$ \cellcolor{green!35} \\\cline{2-9}
wine.2 &  0.10548$^{\phantom{\ddag}}$ \cellcolor{red!35} &  0.04633$^{\phantom{\ddag}}$ \cellcolor{green!21} &  0.05494$^{\phantom{\ddag}}$ \cellcolor{green!13} &  0.04024$^{\phantom{\ddag}}$ \cellcolor{green!27} &  0.05554$^{\phantom{\ddag}}$ \cellcolor{green!12} &  0.03692$^{\phantom{\ddag}}$ \cellcolor{green!30} &  0.03263$^{\dag}$ \cellcolor{green!34} & \textbf{0.03204}$^{\phantom{\ddag}}$ \cellcolor{green!35} \\\cline{2-9}
wine.3 &  0.12182$^{\phantom{\ddag}}$ \cellcolor{red!33} &  0.06949$^{\phantom{\ddag}}$ \cellcolor{green!17} &  0.06729$^{\phantom{\ddag}}$ \cellcolor{green!19} &  0.12294$^{\phantom{\ddag}}$ \cellcolor{red!35} &  0.07350$^{\phantom{\ddag}}$ \cellcolor{green!13} &  0.08203$^{\phantom{\ddag}}$ \cellcolor{green!5} &  0.05549$^{\phantom{\ddag}}$ \cellcolor{green!31} & \textbf{0.05166}$^{\phantom{\ddag}}$ \cellcolor{green!35} \\\cline{2-9}
wine-q-red &  0.22687$^{\phantom{\ddag}}$ \cellcolor{red!28} &  0.21423$^{\phantom{\ddag}}$ \cellcolor{green!4} &  0.21412$^{\phantom{\ddag}}$ \cellcolor{green!4} &  0.21717$^{\phantom{\ddag}}$ \cellcolor{red!3} &  0.20453$^{\ddag}$ \cellcolor{green!29} &  0.20959$^{\ddag}$ \cellcolor{green!16} &  0.22927$^{\ddag}$ \cellcolor{red!35} & \textbf{0.20249}$^{\phantom{\ddag}}$ \cellcolor{green!35} \\\cline{2-9}
wine-q-white &  0.33435$^{\phantom{\ddag}}$ \cellcolor{red!5} &  0.31307$^{\phantom{\ddag}}$ \cellcolor{green!6} &  0.26376$^{\phantom{\ddag}}$ \cellcolor{green!33} &  0.29319$^{\phantom{\ddag}}$ \cellcolor{green!17} &  0.38848$^{\phantom{\ddag}}$ \cellcolor{red!35} &  0.38418$^{\phantom{\ddag}}$ \cellcolor{red!32} & \textbf{0.26069}$^{\phantom{\ddag}}$ \cellcolor{green!35} &  0.27093$^{\phantom{\ddag}}$ \cellcolor{green!29} \\\cline{2-9}
yeast &  0.47094$^{\phantom{\ddag}}$ \cellcolor{red!35} &  0.27772$^{\phantom{\ddag}}$ \cellcolor{green!30} &  0.28420$^{\phantom{\ddag}}$ \cellcolor{green!28} & \textbf{0.26532}$^{\phantom{\ddag}}$ \cellcolor{green!35} &  0.42430$^{\phantom{\ddag}}$ \cellcolor{red!19} &  0.41177$^{\phantom{\ddag}}$ \cellcolor{red!14} &  0.44344$^{\phantom{\ddag}}$ \cellcolor{red!25} &  0.39885$^{\dag}$ \cellcolor{red!10} \\\cline{2-9}
\hline 
 \textit{Average} &  0.26198$^{\phantom{\ddag}}$ \cellcolor{red!35} &  0.23992$^{\phantom{\ddag}}$ \cellcolor{red!17} &  0.26182$^{\phantom{\ddag}}$ \cellcolor{red!34} & \textbf{0.17587}$^{\phantom{\ddag}}$ \cellcolor{green!35} &  0.25255$^{\phantom{\ddag}}$ \cellcolor{red!27} &  0.23828$^{\phantom{\ddag}}$ \cellcolor{red!15} &  0.19214$^{\ddag}$ \cellcolor{green!21} &  0.18541$^{\dag}$ \cellcolor{green!27} \\\cline{2-9}
\textit{Rank} &  6.8 \cellcolor{red!35} &  4.2 \cellcolor{green!15} &  4.8 \cellcolor{green!3} & \textbf{3.2} \cellcolor{green!35} &  5.4 \cellcolor{red!8} &  4.6 \cellcolor{green!7} &  3.3 \cellcolor{green!34} &  3.6 \cellcolor{green!28} \\\hline

\end{tabular}
